OneMax is not the Easiest Function for Fitness Improvements

We study the $(1:s+1)$ success rule for controlling the population size of the $(1,\lambda)$-EA. It was shown by Hevia Fajardo and Sudholt that this parameter control mechanism can run into problems for large $s$ if the fitness landscape is too easy. They conjectured that this problem is worst for the OneMax benchmark, since in some well-established sense OneMax is known to be the easiest fitness landscape. In this paper we disprove this conjecture and show that OneMax is not the easiest fitness landscape with respect to finding improving steps. As a consequence, we show that there exists $s$ and $\varepsilon$ such that the self-adjusting $(1,\lambda)$-EA with $(1:s+1)$-rule optimizes OneMax efficiently when started with $\varepsilon n$ zero-bits, but does not find the optimum in polynomial time on Dynamic BinVal. Hence, we show that there are landscapes where the problem of the $(1:s+1)$-rule for controlling the population size of the $(1, \lambda)$-EA is more severe than for OneMax.

==> efficient_onemax.tex <==
\section{Main proof}

We start this section by defining some helpful notation. Afterwards, we give an informal sketch of the main ideas, before we give the full proof.
\begin{definition}
    Consider the \saolea optimizing a dynamic function \(f = f^t\), and let $Z^t = \ZM(x^t)$. For all times $t$ and all $i\in \ZZ$, we define 
    \begin{align*}
        p^{f,t}_i := \Pr[Z^{t}-Z^{t+1} = i \mid x^t, \lambda^t] \qquad \text{ and } \qquad
        \Delta^{f,t}_i := i \cdot p^{f,t}_i.
    \end{align*}
    We will often drop the superscripts \(f\) and \(t\) when the function and the time are clear from context. We also define \(p_{\ge i} := \sum_{j = i}^{\infty}{p_j}\) and \(\Delta_{\ge i} := \sum_{j=i}^\infty{\Delta_j}\); both \(p_{\le i}\) and \(\Delta_{\le i}\) are defined similarly. Finally, we write
    \begin{align*}
        \Delta^{f,t}  := \EE[Z^{t}-Z^{t+1} \mid x^t, \lambda^t] = \sum\nolimits_{i=-\infty}^\infty \Delta^{f,t}_i.
    \end{align*}
\end{definition}

Note that $i>0$ and $\Delta >0$ corresponds to steps/drift \emph{towards} the optimum and $i<0$ and $\Delta <0$ \emph{away from} the optimum.

\begin{definition}[Improvement Probability, Equilibrium Population Size]\label{def:lambdastar}
    Let \(x \in \{0,1\}^n\) and \(f\) be a strictly monotone function. Let \(y\) be obtained from \(x\) by flipping every bit independently with probability \(1/n\). We define
    \begin{align*}
        \pimp^f(x) := \Pr[ f(y) > f(x) ] \qquad \text{ and }\qquad \qimp^f(x,\lambda) := 1- (1-\pimp^f(x))^\lambda,
    \end{align*}
    as the probability that respectively a single offspring or any offspring improves the fitness of \(x\). We also define the \emph{equilibrium population size} as
    \begin{align}\label{eq:def:lambdastar}
        \lambda^{*, f}(x,s) := \log_{(1 - \pimp^f(x))}\big(\tfrac{s}{1+s}\big).
    \end{align}
    As usual, we drop the superscript when \(f\) is clear from context. As the two functions we consider are symmetric (i.e.\ all bits play the same role) $\pimp$ only depends on $\ZM(x) = \eps n$ so we sometimes write by slight abuse of notation $\pimp(\eps n,s)$ instead of $\pimp(x,s)$, and sometimes we also drop the parameters by writing just $\pimp$ when they are clear from the context \XZ{added this, does it remain in the scope of slight abuse?}, and similarly for $\qimp$ and $\lambda^*$.
    %Moreover, since $\pimp$ only depends on $\eps = \ZM(x)/n$ instead of $x$, we sometimes write by slight abuse of notation $\pimp(\eps,s)$ instead of $\pimp(x,s)$, and similarly for $\qimp$ and $\lambda^*$.
\end{definition}

\begin{remark}\label{rem:equilibrium}
    For all \(x,s\) and \(f\), $\lambda^{*,f}(x,s)$ is chosen to satisfy 
    \begin{align*}
        %1 - (1 - \pimp^f(x))^{\lambda^{*,f}(x,s)} =
        \qimp^f(x,\lambda^{*,f}(x,s)) = \tfrac{1}{s+1}.
    \end{align*}
    Note that the equilibrium population size \(\lambda^{*}\) need not be an integer. Moreover, rounding $\lambda$ to the next integer can change the success probability by a constant factor. Thus we must take the effect of rounding into account. Fortunately, as we will show, the effect of changing the function $f$ from \onemax to \DBV is much larger than such rounding effects. %However, in our case we will show that if \(\lambda\) is a large enough integer and `close' to \(\lambda^*(x)\), then the probability of finding an improvement from search point \(x\) with an offspring population of size \(\lambda\) is `close' to \(1/(1+s)\).
\end{remark}

\subsection{Sketch of Proof}\label{sec:sketch}

We have three quantities that depend on each other: the target population size $\lambda^*$, the target success rate $1/(s+1)$ and the distance $\eps := Z/n$ of the starting point from the optimum. Essentially, choosing any two of them determines the third one. In the proof we will choose $\lambda^*$ and $s$ to be large and $\eps$ to be small. As $\eps$ is small, it is very unlikely to flip more than one zero-bit and the positive contribution to the drift is dominated by the term $\Delta_1$ (Lemma~\ref{lem:approximate_positive_drift}). For \onemax, we also have the other direction: if $\lambda$ is large, then the negative contribution to the drift is dominated by $\Delta_{-1}$ (Lemma~\ref{lem:approximate_negative_drift}). 

The key to the proof is that under the above assumptions, the improvement probability $\pimp$ for \DBV is by a constant factor larger than for \onemax (Lemma~\ref{lem:improvement_single_OM_DBV}). This is not hard to understand. Since it is unlikely to flip more than one zero-bit, the main way to improve the fitness for \onemax is by flipping a single zero-bit and no one-bits. Likewise, \DBV also improves the fitness in this situation. However, \DBV may also improve the fitness if it flips, for example, exactly one zero-bit and one one-bit. This improves the fitness if the zero-bit has higher weight, which happens with probability $1/2$. This already makes $\pimp^{\DBV}$ by a constant factor larger than $\pimp^{\OM}$. (There are even more ways to improve the fitness for \DBV that we don't need to take into account.) As a consequence, for the same values of $s$ and $\eps$, the target population size $\lambda^*$ for \DBV is by a constant factor smaller than for \onemax (Corollary~\ref{cor:equilibrium_OM_DBV}).

This enables us to (mentally) fix some large $\lambda$, choose $\eps$ such that the drift for \onemax at $Z=\eps n$ is slightly positive (towards the optimum) and choose the $s$ that satisfies $\lambda^{*,\OM}(\eps,s) = \lambda$. Here, `slightly positive' means that $\Delta_1 = 4|\Delta_{-1}|$. This may seem like a big difference, but in terms of $\lambda$ it is not. Changing $\lambda$ only affects $\Delta_1$ mildly. But adding just a single child (increasing $\lambda$ by one) reduces $\Delta_{-1}$ by a factor of $\approx 1 - 1/e$, which is the probability that the additional child is not a copy of the parent. So our choice of $\lambda^*, \eps$ and $s$ ensures positive drift for \onemax as long as $\lambda \ge \lambda^*-1$, but not for a much wider range. However, as we show, $\lambda$ stays concentrated in this small range due to our choice of $F=1+o(1)$. This already would yield progress for \onemax in a small range around $Z =\eps n$. To extend this to all values $Z \le \eps n$, we consider the potential function $G^t = Z^t - K\log_F(\lambda^t)$, and show that this potential function has drift towards zero (Corollary~\ref{cor:OM_positive_drift}) whenever $Z >0$, similar to~\cite{hevia2021arxiv,kaufmann2022arxiv}. For $\DBV$, we show that $\lambda$ stays in a range below $\lambda^{*,\DBV}(\eps,s) + 1$, which is much smaller than $\lambda^{*,\OM}(\eps,s)$, and that such small values of $\lambda$ give a negative drift on $Z^t$ (away from the optimum, Lemma~\ref{lem:construction_inefficient_DBV}). Hence, the algorithm is not able to cross the region at $Z=\eps n$ for \DBV.

%\begin{remark}
%    The effect of each bit is symmetric for the two functions \(\OM\) and \(\DBV\) that we consider. In particular this implies that \(\lambda^*(x,s)\) only depends on \(\ZM(x)\) and $s$. In a slight abuse of notation, we will often write \(\lambda^*(Z, s)\).
%\end{remark}

% $p_{i} := \Pr[Z^{t}-Z^{t+1} = i]$ for \onemax.

% $\Delta_{i} := i\Pr[Z^{t}-Z^{t+1} = i]$ for \onemax.

% $\Delta_{\ge i} := \sum_{j\ge i} \Delta_i$ etc.

% $\lambda^*$ denotes the equilibrium point. Depends on $Z^t$ and $s$.

\subsection{Full Proof}

In the remainder of this section, we give the full proof. We start with a lemma saying that $\lambda \le n^2$, and $Z$ never changes by more than $\log n$.

\begin{lemma}\label{lem:small-steps}
Consider the \saolea on \onemax or \dynBV. With probability $1-n^{-\omega(1)}$, either the optimum is found or $\lambda^t \le n^2$ holds for super-polynomially many steps, and in all of these steps $|Z^t-Z^{t+1}| \le \log n$.
\end{lemma}
\begin{proof}
In order to grow above $n^2$, there would need to be a non-improving step when $\lambda^t \ge n^2/F^{1/s}$. Let us call this event $\mathcal E^t$. The probability that a fixed offspring finds an improvement is at least $1/n \cdot (1-1/n)^{n-1} \geq 1/(en)$ (using Lemma~\ref{lem:basic}), even if the algorithm is just one step away from the optimum. Hence, the probability that none of $\lambda^t$ offspring finds an improvement is at most 
\begin{align*}
\Pr[\mathcal E^t] \le  (1-\tfrac{1}{en})^{\lambda^t} \le e^{-(\lambda^t-1)/(en)} = e^{-\Omega(n)}.
\end{align*}
using Lemma \ref{lem:basic} for the second inequality. Even a union bound over a super-polynomial number of steps leaves the error probability $e^{-\Omega(n)}$ unchanged. This proves the first statement.

For the step sizes, condition on $\mathcal E^t$. We can bound the difference $|Z^t-Z^{t+1}|$ from above by the maximal number of bits that any offspring flips. The probability that a fixed offspring flips exactly $k \ge 1$ bits is at most 
\begin{align*}
\binom{n}{k}\Big(\frac{1}{n}\Big)^k(1-1/n)^{n-k} \le \frac{1}{k!},
\end{align*}
and the probability that it flips at least $k$ bits is at most $\sum_{i\ge k} 1/i! \le 2/k!$, since the factorials are bounded by a geometric sum as $1/(k+1)! \le 1/(2\cdot k!)$. For $k = \log n$ this bound is $2/k! = e^{-\Omega(k\log k)} = e^{-\omega(\log n)} = n^{-\omega(1)}$, and the same holds after a union bound over at most $n^2$ offspring, and after a union bound over a super-polynomial (suitably chosen) number of steps.\qed
\end{proof}

In some of our arguments, we use an estimation of \(\pimp^{\OM}\) and \(\pimp^{\DBV}\), which we provide below.

\begin{lemma}
    \label{lem:pimp_roughly_epsilon}
    Let \(f \in \{\OM, \DBV\}\). 
    %We have \(\eps/e \le \pimp^f(\varepsilon) \le \eps\). 
    Then $\pimp^f(\varepsilon) = \Theta(\eps)$.
\end{lemma}

\begin{proof}
    For both functions, a given child improves the fitness if it flips only a zero-bit. For this reason we must have \(\pimp \ge \varepsilon (1 - 1/n)^{(1 - \varepsilon) n } \ge \varepsilon / e\) by Lemma~\ref{lem:basic}.\JL{There is a subtlety here: we need $\eps \ge 1/n$ for the last inequality to hold. And we do have this since $\eps := Z/n \ge 1/n$ for $\eps>0$, and the inequality is trivially true for $\eps =0$. I would rather not make this explicit, unless a reviewer insists.} On the other hand, if the fitness improves then clearly at least a zero-bit must have been flipped meaning that \(\pimp \le \varepsilon\). Thus $\pimp = \Theta(\eps).$ \qed
\end{proof}

The next lemma is one way of stating that \onemax is the easiest function with respect to minimizing the distance from the optimum. Actually, the result would remain true with the same proof if we replaced \(\DBV\) by any other function, or if the algorithm used any other method for offspring creation.

\begin{lemma}
    \label{lem:comparison_positive_drift_OM_DBV}
    %\label{lem:comparison-of-drift}
    %There exist \(\lambda_0 \ge 1\) and \(\varepsilon_0 > 0\) such that the following holds. Let \(\lambda \ge \lambda_0\) and \(\varepsilon < \varepsilon_0\), then 
    For all $\lambda \ge 1$, all $x\in\{0,1\}^n$ and all $i \in \ZZ^+$, 
    \begin{align*}
        \Delta^{\DBV}_{\ge i}(x,\lambda) \le \Delta^{\OM}_{\ge i}(x,\lambda) \quad \text{and} \quad |\Delta^{\DBV}_{\le -i}(x,\lambda)| \ge |\Delta^{\OM}_{\le - i}(x,\lambda)|.
    \end{align*}
    \JL{Slightly rephrased the second inequality to avoid confusion for readers who don't recall the sign. }
\end{lemma}
\begin{proof}
For any $j\in\ZZ$, the event $Z^{t+1} \ge Z^t - j$ can only happen for \onemax if $\ZM(y) \ge \ZM(x) - j$ holds for all offspring $y$ of $x$, since \onemax picks the offspring which minimizes $\ZM(y)$. In this case, regardless of the selection of \DBV, the selected offspring also satisfies $\ZM(y) \ge \ZM(x) - j$. Hence, $p_{\le j}^\OM \le p_{\le j}^{\DBV}$ and 
%\begin{align}\label{eq:compare-p-OM-DBV}
    $p_{\ge j}^\OM \ge p_{\ge j}^{\DBV}$
%\end{align} 
for all $j \in \ZZ$. In particular, for all \(i \ge 0\)
\begin{align*}
    \Delta_{\le -i}^{\OM} &= -i \cdot p_{\le -i}^{\OM} - \sum\nolimits_{j=-\infty}^{-i-1} p_{\le j}^{\OM} \ge -i \cdot p_{\le -i}^{\DBV} - \sum\nolimits_{j=-\infty}^{-i-1} p_{\le j}^{\DBV}  = \Delta_{\le -i}^{\DBV},
\end{align*}
and
\begin{align*}
    \Delta_{\ge i}^{\OM} &= i \cdot p_{\ge i}^{\OM} + \sum\nolimits_{j=i+1}^{\infty} p_{\ge j}^{\OM} \ge i \cdot p_{\ge i}^{\DBV} + \sum\nolimits_{j=i+1}^{\infty} p_{\ge j}^{\DBV}  = \Delta_{\ge i}^{\DBV}.\qquad \qed
\end{align*}%\qed
\end{proof}


%  \begin{lemma}\label{lem:comparison-of-drift}
%      There exist constants \(\lambda_0, c > 0\) such that the following holds for all $\lambda \ge \lambda_0$. Assume that \(x,\lambda\) satisfy \(p^{\OM}_{\ge 1}(x) \le 1/2\). Then 
%      \begin{align*}
%          |\Delta_{\le -1}^{\DBV}| \ge |\Delta_{\le -1}^{\OM}| + c \Delta_{1}^{\OM}.
%      \end{align*}
%      % $\exists c>0, \lambda_0: \forall \lambda \ge \lambda_0$: If $p_{\ge 1} \le 1/2$ then $|\Delta_{\le -1}^{\DBV}| \ge |\Delta_{\le -1}^{\OM}| + c \Delta_{1}^{\OM}$. (Assume $Z^t \le n/2$ or similar if necessary.) 
%  \end{lemma}
%\begin{proof}[of Lemma~\ref{lem:negative_drift_OM_DBV}]
%
%Using the assumed bound $p_{\ge 1} \le 1/2$, it holds that \[c \cdot \Delta_{1}^{\OM}= c \cdot 1 \cdot \Pr[Z^{t}-Z^{t+1} = 1] \le c \cdot p_{\ge 1} \le c/2\] so it suffices to prove \[ |\Delta_{\le -1}^{\DBV}| \ge |\Delta_{\le -1}^{\OM}| +c/2.\]
%\JL{Added the $+c/2$ on the right hand side, otherwise it does not make sense to me.}
%Note that the left-hand side describes the absolute value of the expected \ZM-drift for \dynBV, conditional on a \ZM-increase of at least $1$, the right-hand side analogous for the \onemax-function.  \par
%It suffices to prove that for every $i \le -1$, \JL{This doesn't hold. But what does hold is $p^\DBV_{\le i} \ge p^\OM_{\le i}$ and $\Delta^\DBV_{\le i} \ge \Delta^\OM_{\le i}$. We want to use it with $i=-2$ and use that to show that $\Delta^\DBV_{\ge -1} \ge \Delta^\DBV_{\le -1} +c/2$, where the $+c/2$ comes from cases in which a single zero-bit and two one-bits are flipped.}
%
%The (new) statement of the lemma is simply:
%\[\Pr^{\DBV}[Z^{t}-Z^{t+1}=-1]\ge \Pr^{\OM}[Z^{t}-Z^{t+1}=-1]\]
%If a generation contains a copy of the parent, \[\Pr^{\OM}[Z^{t}-Z^{t+1}=-1]=0\]
%Hence we can upper-bound the right-hand side by the probability that we do not encounter such a copy. By Lemma 12 from \cite{kaufmann2022arxiv}, 
%\[e^{-b_1 \lfloor \lambda \rceil}  \ge \Pr^{\OM}[Z^{t}-Z^{t+1}=-1]\]
%for some constant $b_1$. A sufficient condition for the event $Z^{t}-Z^{t+1}=-1$ for $\dynBV$ is that all offspring  flip exactly 1 one-bit and no zero-bit. Denote this event by $Q$. Then
%\[\Pr[Q]=(\frac{n-Z^t}{n})^{\lfloor \lambda \rceil}= (1-\eps)^{\lfloor \lambda \rceil}\]
%Now choosing $\eps_0 \le 1-e^{-b_1 \lfloor \lambda \rceil}$ finishes the proof.
%\MK{Okay here we still need to account for the probabilities of not flipping the other bits, but this will only change the result by a constant factor. Okay the constant factors break the proof :( Need to do something smarter. TODO}
%\[\Pr[Q]=((\frac{n-Z^t}{n})(1-\frac{1}{n})^{Z^t})(1-\frac{1}{n})^{n-Z^t-1})^{\lfloor \lambda \rceil} \ge (\frac{(1-\eps)^2}{e})^{\lfloor \lambda \rceil}\]
%Note that a necessary condition of the event $Z^{t}-Z^{t+1}=-1$ for $\OM$ is that all offspring flip at least one one-bit. Denote this event by $A$. This condition is also sufficient for $Z^{t}-Z^{t+1}\le -1$ for $\dynBV$, so we have
%\[\Pr^{\DBV}[Z^{t}-Z^{t+1}\le -1]\ge \Pr[A] \ge \Pr^{\OM}[Z^{t}-Z^{t+1}=-1]\]
%\[|i \cdot \Pr^{\DBV}[Z^{t}-Z^{t+1}=i]| \ge |i \cdot \Pr^{\OM}[Z^{t}-Z^{t+1}=i]| \] 
%and there exists an $i_0 \le -1$ such that
%\[|i_0 \cdot \Pr^{\DBV}[Z^{t}-Z^{t+1}=i_0]| > |i_0 \cdot \Pr^{\OM}[Z^{t}-Z^{t+1}=i_0]| \]
%The two conditions are equivalent to
%\[\Pr^{\DBV}[Z^{t}-Z^{t+1}=i] \ge \Pr^{\OM}[Z^{t}-Z^{t+1}=i] \forall i \le -1\]
%and for some $i_0\le -1$
%\[\Pr^{\DBV}[Z^{t}-Z^{t+1}=i_0] > \Pr^{\OM}[Z^{t}-Z^{t+1}=i_0]\]
%Denote the probability of having a copy of the parent in the offspring population We know that for $i\le -1$ $\Pr^{\OM}[Z^{t}-Z^{t+1}=i|\overline{A}]$ Lemma 12 from \cite{kaufmann2022arxiv} tells us that
%For \onemax, a necessary condition for a \ZM-increase of $i$ bits is that all $\lfloor \lambda \rceil$ flip at least $i$ one-bits:
%\[\Pr^{OM}[Z^{t}-Z^{t+1}=i] \le (\sum_{j=i}^{n-Z^t}\binom{n-Z^t}{j}(\frac{1}{n})^{j}) ^{\lfloor \lambda \rceil} \]
%\MK{in progress, for \onemax, a necessary condition for a \ZM-increase is the absence of a copy of a parent,...}\par
%Denote by $A_{>i}^\DBV$ the event that, for \dynBV, $Z^t-Z^{t+1}>i$ and analogously  $A_{>i}^\OM$. 
%Then \[A_{>i}^\DBV \implies A_{>i}^\OM\]. Therefore \[p^\DBV_{> i} \le p^\OM_{> i}\] and hence \[p^\DBV_{\le i}=1-p^\DBV_{> i} \ge 1- p^\OM_{> i}= p^\OM_{\le i}\]
%Now assume $i\le -1$: \[|\Delta^\DBV_{\le i}|=|- \sum_{i\ge 1}p^\DBV_{\le -i}| \ge  |- \sum_{i\ge 1}p^\OM_{\le -i}|= |\Delta^\OM_{\le i}|\]
%\MK{Still need to account for the $\frac{c}{2}$-term. If we have a copy of the parent, the probability of which is increasing exponentially in $\lambda$ by Lemma 12 from the other paper, there will be no $\ZM$-increase for $\onemax$. But if we flip two one-bits and one 0-bit that is highly significant, there will be an increase of at least 1 in the \ZM-term for \dynBV,..} \par
%Let $D:=|\Delta_{\le -1}^{\DBV}|-|\Delta_{\le -1}^{\OM}|$. The claim now follows for any choice of $c\le 2 \cdot D$.  
%\qed
%\end{proof}



%\XZ{I will try to prove the following lemma}
%\begin{lemma}\label{lem:lambdastar-smooth-in-s}
%    \ML{I think we need something stronger...}\JL{This is only meant to be used to apply Lemma \ref{lem:Delta-plus-2}. That lemma needs an \emph{upper} bound on $\lambda$ to be true, but it can be a very weak upper bound.}
%    Decreasing $s$ by $1-c/2$ increases $\lambda^*$ by at most a factor $10$. (Make $c$ smaller if necessary. Assume $\lambda$ suff large, $s$ suff large, $Z^t$ suff small if necessary.)
%    
%    Make sure the following lemmas all hold when we increase $\lambda$ by a factor of $20$ or so.
%\end{lemma}
%\begin{proof}
%The following conditions must be met
%\begin{align*}
%    1 - \frac{C}{2} > \frac{e^{1.5 \eps}-1}{e^{9.5/(e \eps)}-1}, \text{and} (1-C/2)^{-1} (e^{9.5/(e \eps)}-1)^{-1} < s < (e^{1.5 \eps} -1)^{-1}, 
%\end{align*}
%where $\eps = Z^t / n$.
%\qed
%\end{proof}

% \begin{lemma}\label{lem:Delta-minus-2}
%      $\forall \delta \exists \lambda_0$ such that for all $\lambda \ge \lambda_0$ and $Z^t \le n/2$: $|\Delta^\OM_{\le -2}| \le \delta p_{-1}$.
% \end{lemma}

The next lemma states that the negative contribution to the drift for \onemax is dominated by $\Delta_{-1}^{\OM}$. Afterwards, we give an approximate formula for $\Delta_{-1}^{\OM}$.

\begin{lemma}
    \label{lem:approximate_negative_drift}
    \label{lem:Delta-minus-2}
    For every \(\delta > 0\) there exists \(\lambda_0\) such that for all \(\lambda > \lambda_0\) and $\eps \le 1/2$, 
    \begin{align*}
        |\Delta^{\OM}_{\le -2}(\eps n,\lambda)| \le \delta |\Delta^{\OM}_{-1}(\eps n,\lambda)|.
    \end{align*}
\end{lemma}

\begin{proof}
We will show the statement $|\Delta^{\OM}_{\le -2}(\eps n,\lambda)| \le \delta p^{\OM}_{\le -1}(\eps n,\lambda)$, with $\le -1$ on the right hand side. Then the statement in the lemma follows immediately (with a slightly different $\delta$) from $p^{\OM}_{\le -1}(\eps n,\lambda) \le |\Delta^{\OM}_{\le -1}(\eps n,\lambda)| = |\Delta^{\OM}_{-1}(\eps n,\lambda)| + |\Delta^{\OM}_{\le -2}(\eps n,\lambda)|$. 

For $i \ge 1$, let $q_{\ge i}$ be the probability that a fixed offspring flips at least $i$ more one-bits than zero-bits. A necessary condition for that is that at least $i$ bits are flipped. The probability that exactly $i$ bits are flipped is at most $1/i!$, so $q_{\ge i} \le \sum_{j\ge i}1/j! \le 2/i!$. Now consider the event that an offspring flips a single one-bit and no zero-bit. This is counted in $q_{\ge 1}$, but not in $q_{\ge 2}$, and it has probability at least $1/(2e)$. Hence, $q_{\ge 1} \ge q_{\ge 2} + 1/(2e)$. 

The event that $Z^t - Z^{t+1} = -i$ for \onemax implies that all offspring flip at least $i$ more one-bits than zero-bits. Hence,
\begin{align*}
    |\Delta_{-i}^{\OM}| = i \Pr[Z^{t}- Z^{t+1} = -i] \le i (q_{\ge i})^{\rlbd}.
\end{align*}
We use two different ways to bound $q_{\ge i}$. For $i\ge 6$, we have $q_{\ge i} \le 2/i! \le 1/(4ei^2)$, which implies $|\Delta_{-i}^{\OM}| < 1/(4ei)^{\rlbd}$, and $\sum_{i=6}^{\infty}|\Delta_{-i}^{\OM}| < (1/(4e))^{\rlbd}$. For $2\le i\le 5$, we use that $|\Delta_{-i}^{\OM}| < 5(q_{\ge 1} -1/(2e))^{\rlbd}$. Both terms become arbitrarily small compared to $p^{\OM}_{\le -1}(\eps n,\lambda) = (q_{\ge 1})^{\rlbd}$ for $\lambda$ sufficiently large. This concludes the proof.\qed

%For $i \ge 1$, let $q_i$ be the probability that an offspring flips exactly $i$ one-bits, and similarly for $q_{\ge i}$.\JL{There is a bug here. The sum $\sum q_j$ is not meaningful with this definition, for that we would need the probability that all offspring flip \emph{at least} $i$ one-bits (then $\sum q_j$ overcounts, but that should be no problem). \XZ{Oh yes, I see, will try to fix this}} We have
%\begin{align*}
%    q_i = \binom{n-Z^t}{i} \frac{1}{n^i} \Big( 1- \frac{1}{n}\Big)^{n-Z^t-i},
%\end{align*}
%and 
%\begin{align*}
%    q_{\ge i} = \sum_{j=i}^{\infty} q_j \le 2 q_i,
%\end{align*}
%since 
%\begin{align*}
%    \frac{q_{i+1}}{q_i} =  \frac{n-Z^t-i}{i+1} \frac{1}{n-1} \le \frac{1}{2}.
%\end{align*}
%The event that $Z^t - Z^{t+1} = -i$ for \onemax implies that all offspring flip at least $i$ one-bits, since otherwise we would have $Z^t - Z^{t+1} > -i$. Therefore,
%\begin{align*}
%    \Pr[Z^{t}- Z^{t+1} = -i] \le (2 q_i)^{\rlbd},
%\end{align*}
%and
%\begin{align*}
%    |\Delta^{\OM}_{\le -2}| = \sum_{j=2}^{\infty} j \cdot \Pr[Z^t -Z^{t+1}=-j] \le \sum_{j=2}^{\infty} j \cdot (2 q_j)^{\rlbd}.
%\end{align*}
%For all $j \ge 2$, it holds that
%\begin{align*}
%    \frac{(j+1) \cdot (2 q_{j+1})^{\rlbd}}{j \cdot (2 q_j)^{\rlbd}} \le \frac{3}{2} \cdot \frac{1}{2^{\round{\lambda}}},
%\end{align*}
%so we obtain
%\begin{align*}
%    |\Delta^{\OM}_{\le -2}| \le  \frac{ 2 (2 q_2)^{\rlbd}}{1 - \frac{3}{2 \cdot 2^{\round{\lambda}}}} \le 8 (2 q_2)^{\rlbd}.
%\end{align*}
%On the other hand, a sufficient condition for $Z^t - Z^{t+1} = -1$ is that every offspring flips exactly 1 one-bit and 0 zero-bits. So
%\begin{align*}
%    \Pr[Z^t - Z^{t+1} = -1] \ge& \bigg( \binom{n-Z^t}{1} \frac{1}{n} \Big(1- \frac{1}{n}\Big)^{n-1}\bigg)^{\round{\lambda}} = \bigg(q_1 \Big(1-\frac{1}{n}\Big)^{Z^t} \bigg)^{\rlbd} \\
%    \ge& (1-\frac{1}{n})^{Z^t \rlbd} (2 q_2)^{\rlbd}.
%\end{align*}
%\qed
\end{proof}

\begin{lemma}
    \label{lem:strong_approximate_negative_drift}
    For every \(\delta > 0\), there exists \(\lambda_0\) such that the following holds. For every integer \(\lambda > \lambda_0\), there exists \(\varepsilon_0 > 0\) such that for all \(\varepsilon < \varepsilon_0\) we have 
    \begin{align*}
        |\Delta_{\le -1}^{\OM}(\eps n,\lambda)| = (1 \pm \delta)(1 - e^{-1})^{\lambda}.
    \end{align*}
    Additionally, \(\varepsilon_{0}(\lambda) = \Omega(\delta / \lambda)\).
\end{lemma}

\begin{proof}
    Without loss of generality we assume that \(\delta < 1\) and let \(\delta' = \delta /3 \). We assume that \(\lambda\) is sufficiently large so that Lemma~\ref{lem:approximate_negative_drift} can be applied with \(\delta'\).
    
    Clearly, if every child flips at least a one-bit and no zero-bit, then \(Z^t\) must increase. Hence we have 
    \begin{align*}
        |\Delta_{\le -1}| 
            &\ge \left( (1 - (1 - 1/n)^{(1-\varepsilon) n}) \cdot (1 - 1/n)^{\varepsilon n} \right)^{\lambda}\\
            &= (1 - e^{-1} + O(\varepsilon))^\lambda \numberthis \label{eq:lem:strong_approximate_negative_drift_1}
    \end{align*}
    % If the number of zero-bits \(Z^t\) increases, it must be that every child has changed a one-bit to a zero-bit. For this reason
    % \begin{align*}
    %     |\Delta_{\le -1}| 
    %         &\ge \left( 1 - (1 - 1/n)^{(1-\varepsilon) n} \right)^{\lambda} \\
    %         &\ge \left( 1 - e^{\varepsilon - 1} \right)^{\lambda} = (1 - e^{-1} + O(\varepsilon))^\lambda. \numberthis \label{eq:lem:strong_approximate_negative_drift_1}
    % \end{align*}

    For the other direction, $Z^t$ can only increase if every child flips strictly more one-bits than zero-bits. Therefore, 
    \begin{align*}
        |\Delta_{-1}|
            &\le p_{\le -1} 
            \le \left( \sum_{i=0}^{\varepsilon n}{ \binom{\varepsilon n}{i} n^{-i} \tilde{p}_{\ge i+1}  }  \right)^\lambda,
    \end{align*}
    where \(\tilde{p}_{\ge i}\) denotes the probability that a single child flips at \emph{least} \(i\) one-bits.
    
    Now using 
    \begin{align*}
        \tilde{p}_{\ge 1} = 1 - (1 - 1/n)^{(1-\varepsilon) n} \le 1 - e^{-1} \quad \text{and} \quad \tilde{p}_{\ge i} \le {\binom{(1 - \varepsilon)n}{i}} n^{-i} \le 1/2,
    \end{align*}
    when \(i > 1\) and replacing in the display above, we get 
    \begin{align*}
        |\Delta_{-1}| \le (1 - e^{-1} + O(\varepsilon))^{\lambda}. \numberthis \label{eq:lem:construction_equilibrium_OM_2}
    \end{align*}
    
    We may now combine \eqref{eq:lem:strong_approximate_negative_drift_1}, \eqref{eq:lem:construction_equilibrium_OM_2} with Lemma~\ref{lem:approximate_negative_drift} we see that 
    \begin{align*}
        |\Delta_{\le -1}| = (1 \pm \delta')(1 - e^{-1} + O(\varepsilon))^\lambda = (1 \pm \delta') ( 1 - e^{-1} )^\lambda \cdot (1 + O(\varepsilon))^\lambda.
    \end{align*}
    Letting \(\varepsilon_0 = c\delta' / \lambda\) for a sufficiently small absolute constant \(c\), we see that for any \(\varepsilon < \varepsilon_0\) the last term is \(1 \pm \delta'\). For such a \(\varepsilon\) we find 
    \begin{align*}
        |\Delta_{\le -1}| \le (1 \pm 3 \delta') (1 - e^{-1})^\lambda \le (1 \pm \delta) (1 - e^{-1})^\lambda,
    \end{align*}
    which proves the claim.
    
    \qed
\end{proof}

For the positive part of the drift, large steps are negligible for either function when compared to steps of size one for \onemax. The reason why this also holds for \DBV is that \onemax maximizes the drift of $Z$ (towards zero) by always choosing the offspring that provides the best progress in terms of $Z$. Afterwards, we show a bound for 
$\Delta^{\DBV}_1$ in terms of $\Delta^{\OM}_1$ that holds for similar reasons.

\begin{lemma}
    \label{lem:approximate_positive_drift}
    Let \(f \in \{\OM, \DBV\}\). For every \(\delta > 0\) and \(\lambda \ge 1\), there exists \(\varepsilon_0 > 0\) such that for all \(\varepsilon < \varepsilon_0\) we have 
    \begin{align*}
        \Delta_{\ge 2}^f(\eps n,\lambda) \le \delta \Delta_1^{\OM}(\eps n,\lambda).
    \end{align*}
    Note that the right hand side is the drift with respect to \onemax, not to $f$. Additionally we have \(\varepsilon_0(\lambda) = \Omega( \delta/\lambda )\).
\end{lemma}

\begin{proof}
    
    We will first assume $f=\OM$. Consider a given offspring. For any \(i\) zero-bits, there is probability \(n^{-i}\) that they all flip to one-bits. By union bound over \({\varepsilon n \choose i} \le (\varepsilon n)^i / i!\) such choices, the probability that at least \(i\) zero-bits are flipped is at most \(\varepsilon^i/i!\). 
    Now union bounding over all children we find 
    \begin{align*}
        p_{\ge i} = \Pr[Z^t-Z^{t+1} \ge i] \le \lambda \varepsilon^i / i!.
    \end{align*}
    In turn this implies 
    \begin{align*}
        \Delta_{\ge 2} \; \le \; \sum_{i = 2}^\infty{ i p_{\ge i} } \; \le \; 2 \lambda \varepsilon^2.
    \end{align*}
    As a single child flipping exactly a zero-bit and no one-bit implies that \(Z^t\) decreases, we must also have
    \begin{align*}
        \Delta_1 = p_{1} \ge \varepsilon (1 - 1/n)^{n-1} \ge e^{-1} \varepsilon,
    \end{align*}
    by Lemma~\ref{lem:basic}. Choosing \(\varepsilon_0 = \delta/(2e\lambda)\) ensures that \(\Delta_{\ge 2} \le \delta \Delta_1\),
    % We have shown $\Delta_{\ge 2}^{\OM} \le \delta \Delta_1^{\OM}$, 
    and the corresponding bound for $\Delta_{\ge 2}^{\DBV}$ follows from Lemma~\ref{lem:comparison_positive_drift_OM_DBV}.
    
    % We will first assume $f=\OM$. The event that $Z^t -Z^{t+1} = i$ for $i \ge 1$ indicates that the fittest offspring flips $i$ more zero-bits than one-bits, thus implying that all offspring flip at least $i$ more zero-bits than one-bits. Therefore, let $q_i$ denote the probability that a fixed offspring flips exactly $i$ more zero-bits than one-bits, and similarly for $q_{\ge i}$. Then
    % \begin{align*}
    %     p_i = \Pr[Z^t-Z^{t+1} = i] \le q_{\ge i}^{\rlbd}.
    % \end{align*}
    % Let $q_{i, j}$ denote the probability of flipping $i$ one-bits and $j$ zero-bits, then
    % \begin{align*}
    %     q_i = \sum_{j=0}^{\infty} q_{j, j+i} \le 2 q_{0, i},
    % \end{align*}
    % where the last inequality holds as
    % \begin{align*}
    %     \frac{q_{j+1, j+1+i}}{q_{j, j+i}} = \frac{n-Z^t-j}{j+1} \frac{1}{n-1} \frac{Z^t-i-j}{i+j+1} \frac{1}{n-1} \le \frac{1}{2}
    % \end{align*}
    % for all $i \ge 1$ and $j \ge 0$. So
    % \begin{align*}
    %     q_{\ge i} = \sum_{j=i}^{\infty} q_j \le 2 \sum_{j=i}^{\infty} q_{0, j} \le 4 q_{0 ,i},
    % \end{align*}
    % since for $i \ge 1$,
    % \begin{align*}
    %     \frac{q_{0, i+1}}{q_{0, i}} = \frac{Z^t - i}{i+1} \frac{1}{n-1} \le \frac{1}{2}.
    % \end{align*}
    % To bound $\Delta_{\ge 2}$, we have
    % \begin{align*}
    %     \Delta_{\ge 2} = \sum_{i=2}^{\infty} i \cdot p_i \le \sum_{i=2}^{\infty} i \cdot (4 q_{0, i})^{\rlbd} \le 2 (4 q_{0, 2})^{\rlbd} \frac{1}{1-\frac{3}{2} \frac{1}{2^{\rlbd}}} \le 8 (4 q_{0, 2})^{\rlbd}, 
    % \end{align*}
    % as for $i \ge 2$,
    % \begin{align*}
    %     \frac{(i+1) (4 q_{0, i+1})^{\rlbd}}{i (4 q_{0, i})^{\rlbd}} \le \frac{i+1}{i} \frac{1}{2^{\rlbd}} \le \frac{3}{2}. \frac{1}{2^{\rlbd}} 
    % \end{align*}
    
    % On the other hand, a sufficient condition for $Z^t -Z^{t+1} = 1$ is that every offspring flips 1 zero-bit and no one-bit, so we have $p_1 \ge q_{0, 1}^{\rlbd}$ and thus $\delta \Delta_1 \ge \delta q_{0, 1}^{\rlbd}$. To ensure $\Delta_{\ge 2} \le \delta \Delta_1$, we show that the lower bound of $\Delta_{\ge 2}$ is smaller or equal to the upper bound of $\delta \Delta_1$, namely 
    % \begin{align*}
    %     8 (4 q_{0, 2})^{\rlbd} \le \delta q_{0, 1}^{\rlbd}.
    % \end{align*}
    % Since for $Z^t = \eps n < \eps_0 n $,
    % \begin{align*}
    %     \frac{q_{0, 2}}{q_{0, 1}} = \frac{\binom{Z^t}{2} \frac{1}{n^2} (1-\frac{1}{n})^{Z^t -2}}{\binom{Z^t}{1} \frac{1}{n} (1-\frac{1}{n})^{Z^t -1}} = \frac{Z^t-1}{2} \frac{1}{n-1} < \eps_0,
    % \end{align*}
    % if we pick $\eps_0 < \delta/32$, the desired inequality holds. 
    % So we have shown $\Delta_{\ge 2}^{\OM} \le \delta \Delta_1^{\OM}$, and the corresponding bound for $\Delta_{\ge 2}^{\DBV}$ follows from Lemma~\ref{lem:comparison_positive_drift_OM_DBV}.



%    , we can use it to show a similar equation for \DBV. If for \DBV, $Z^t - Z^{t+1} \ge i$, this implies $Z^t - Z^{t+1} \ge i$ for \OM, since \OM minimizes $Z^{t+1}$. Therefore,
%    \begin{align*}
%        \Delta_{\ge 2}^{\DBV} = \sum_{i=2}^{\infty} p_{\ge i}^{\DBV} \le \sum_{i=2}^{\infty} p_{\ge i}^{\OM} = \Delta_{\ge 2}^{\OM} \le \delta \Delta_1^{\OM}.
%    \end{align*}
%    On the other hand, 
%    \begin{align*}
%        \Delta_1^{\OM} = p_1^{\OM} \le p_{\le 1} ^{\OM} \le p_{\le 1}^{\DBV} = \Delta_1^{\DBV} + \Delta_{\le -1}^{\DBV} = (1+\delta') \Delta_1^{\DBV}
%    \end{align*}
%    holds for some positive constant $\delta'$ \XZ{Is there an easy way to show this?}. Similar as before, we enforce the lower bound of $\delta \Delta_1^{\DBV}$ is at least the upper bound of $\Delta_{\ge}^{\DBV}$, namely
%    \begin{align*}
%        \frac{\delta}{1+\delta'} \Delta_1^{\OM} \ge \Delta_{\ge 2}^{\OM},
%    \end{align*}
%    which holds if we pick $\eps_0 < \delta /(1+\delta')/32$.
    \qed
\end{proof}



% \begin{lemma}\label{lem:Delta-plus-2}
%      $\forall s \exists \eps_0\forall \eps \le \eps_0$: If $\lambda^*(s) \le \lambda \le 20 \lambda^*(s)$ and $Z^t = \eps n$ then $|\Delta_{\ge 2}| \le \delta p_{1}$.
% \end{lemma}

%\ML{I think we don't need the proposition commented out below, so I killed it.}
% \begin{proposition}\label{prop:drift}
% There are $s,\eps$ such that for $Z^t = \eps n$,
% \begin{enumerate}
%     \item $\Delta^t_{\OM}(s,Z^t,\lambda^*(s,Z^t)) \ge cs_0$, and
%     \item $\Delta^t_{\DBV}(s,Z^t,\lambda^*(s,Z^t)) \le - cs_0$.
% \end{enumerate}
% \JL{It would be convenient for later to show the slightly stronger bound $\Delta \ge p_1 + \Delta_{\le -1} \ge p_1 - \sum_{i=1}^{\infty}i \Pr(\text{all offspring flip at least $i$ bits}) \ge cs_0$ for \onemax. Then it becomes trivial that the drift (or the lower bound on the right hand side) increases at $\lambda^*(\eps)$ as $\eps$  decreases, since the positive term $p_1 = 1/(s+1)$ stays constant (up to rounding of $\lambda$), and the negative terms are decreasing with $\lambda$.}
% \end{proposition}

% \begin{proof}
% Choose $\delta = c/10$ or so. Then pick $\lambda = \lambda_0$ from third lemma and $\eps = \eps_0$ from fourth lemma. Then $\Delta_{\ge 2}$  and $\Delta_{\le -2}$ are negligible. Choose $s_0$ such that the drift for \onemax is zero for this $\lambda,\eps$. 

% Now choose $s := s_0(1-c/2)$. This increases $\lambda^*$ by at most a factor of $10$, so all lemmas are still applicable. Then the drift is of order $+ c s_0$ for \onemax and of order $- cs_0$ for \DBV by first lemma. 

% \end{proof}

\begin{lemma}
    \label{lem:positive_drift_OM_DBV}
    For every \(\lambda \ge 1\) and \(\delta > 0\), there exists \(\varepsilon_0 > 0\) such that for all \(\varepsilon < \varepsilon_0\) we have 
    \begin{align*}
        \Delta^{\DBV}_1(\eps n,\lambda) \le (1 + \delta) \Delta^{\OM}_1(\eps n,\lambda).
    \end{align*}
    Additionally we have \(\varepsilon_0(\lambda) = \Omega( \delta/\lambda )\).
    %\ML{Maybe I don't need the \(\delta\)...}
\end{lemma}

\begin{proof}
    We may assume $\lambda \eps_0 \le e$. 
    Let $\tilde p_{\ge 2}$ be the probability that a fixed offspring flips at least $2$ zero-bits, and let $\tilde q_{\ge 2}$ be the probability that there exists such an offspring. Then $\tilde p_{\ge 2} \le \eps^2$, and by a union bound $\tilde q_{\ge 2} \le \lambda \eps^2$. 
    %, and hence $\Delta_{\ge 2}^{\DBV} \le 2 \tilde p_2 + \sum_{i\ge 3} \tilde p_i \le 3 \eps^2$ if $\eps_0$ is sufficiently small. 
    On the other hand, assume that no offspring flips at least two zero-bits and that $Z^{t+1} = Z^t -1$ for \DBV. Then the selected offspring must have exactly one zero-bit and no one-bit flipped. In this case, this offspring (or an equivalent one) is also selected for \onemax. Therefore, $\Delta_1^{\DBV} \le \Delta_1^{\OM} + \tilde q_{\ge 2}$. 
    
    Let $p_{0,1}$ be the probability that there is an offspring that flips exactly one zero-bit and no one-bit. For each offspring, this happens with probability at least $\eps/e$, so 
    \begin{align*}
        \Delta_{\ge 1}^{\OM} \ge p_{0,1} \ge 1-(1-\eps/e)^{\lambda} \stackrel{\text{Lem }\ref{lem:basic}}{\ge} \frac{\lambda \eps/e}{1+\lambda \eps/e} \ge \frac{\lambda \eps}{2e}. 
    \end{align*}  
    In particular, this implies $\tilde q_{\ge 2} \le \lambda \eps^2 \le 2e \eps \Delta_{\ge 1}^{\OM}$. 
    Combining this with $\Delta_{\ge 2}^{\OM} \le \delta' \Delta_1^{\OM}$ for an arbitrary choice of $\delta'>0$ by Lemma~\ref{lem:approximate_positive_drift}, we obtain
    \begin{align*}
        \Delta_1^{\DBV} \le \Delta_1^{\OM} + \tilde q_{\ge 2} \le (1+2e\eps)\Delta_{\ge 1}^{\OM} \le (1+2e\eps)(1+\delta')\Delta_1^{\OM}.
    \end{align*}
    Choosing $\delta'$ and $\eps$ small enough finishes the proof.\qed
\end{proof}



%\begin{lemma}\label{lem:close-to-lambdastar}
%Let $s >0$ be constant, let $f$ be either \onemax or \DBV and let $F=1+\eta$ for some $\eta \in o(1/(\sqrt{n}\log^2 n)) \cap \omega(\log n /n)$. Assume that $\lambda^{t_0} \le n^2$ and $Z^{t_0} =\eps n$ for some time $t_0$ and some $\eps \ge n/\log^2 n$. Then there exists $\tau \in O(\eta^{-1}\log n)$ such that the following holds with probability $1-n^{-\omega(1)}$.
%\begin{enumerate}
%    \item $\lambda^{t_1} = \lambda^*(\eps n,s) \pm 1/2$ for %    \item Let $t_2 \in [t_1,t_1+n^2]$ denote the earliest point in time when $|Z^{t_2}-\eps n| \ge n/\log^3 n$, and $t_2 := t_1 +n^2$ if no such time exists. Then $\lambda^t = \lambda^*(\eps n,s) \pm 1/2$ for all $t\in [t_1,t_2]$.
%\end{enumerate}
%\end{lemma}

We also use that $\lambda^*$ changes smoothly in $\eps$.

\begin{lemma}
    \label{lem:lambda_changes_slowly}
    Let \(f \in \{\OM, \DBV\}\). For all \(\varepsilon, s,\rho > 0\) there exists \(\eps'>0\) and $n_0\in \NN$ such that for all $n\ge n_0$,
    \begin{align*}
        \lambda^{*, f}((\varepsilon - \eps')n, s) - \lambda^{*, f}((\varepsilon + \eps')n, s) \le \rho.
    \end{align*}
\end{lemma}
\begin{proof}
    This is a simple consequence of the definition: 
    \begin{align*}
        \lambda^{*,f}(Z, s) = \log_{1 - \pimp(Z)}(s/(s+1)) = \frac{\log(s/(s+1))}{\log(1 - \pimp(Z))}.
    \end{align*}
    Recall that by Lemma~\ref{lem:pimp_roughly_epsilon} we have \(\pimp(Z) =\Theta(Z/n)\), so increasing or decreasing it by \(\eps' n\) for a small \(\eps'>0\) changes \(\pimp\) only by a small constant. Choosing \(\eps'\) sufficiently small, we can guarantee that $\lambda^{*,f}(Z, s)$ changes by at most \(\rho\).\qed
\end{proof}

We are finally ready for the key step in the next two lemmas, which is that the success probability for \onemax is substantially smaller than for \DBV. This means that \DBV is easier than \onemax with respect to fitness improvements.


\begin{lemma}
    \label{lem:improvement_single_OM_DBV}
    There exists \(\varepsilon_0, \alpha > 0\) such that for all \(\varepsilon < \varepsilon_0\), we have 
    \begin{align*}
        \pimp^{\OM}(\eps n) \le ( 1 - \alpha ) \pimp^{\DBV}(\eps n).
    \end{align*}
\end{lemma}

\begin{proof}
    Let $E_{i,j}$ denote the event that exactly $i$ one-bits and $j$ zero-bits are flipped, and let $\tilde E_j$ be the event that $j$ zero-bits are flipped. We write $q_{i,j}:= \Pr(E_{i,j})$ and $\tilde p_j := \Pr(\tilde E_j)$, and we define $\tilde p_{\ge j}$ analogously. 
    Observing that \(p_j = {\binom{\varepsilon n}{j}} n^{-j} (1 - 1/n)^{\varepsilon n - j}\), we compute  
    \begin{align*}
        \tilde{p}_{j+1} = \tilde{p}_j \; \frac{\varepsilon n - j}{j+1} \frac{1}{n \cdot (1 - 1/n)} \le \tilde{p}_j / 2,
    \end{align*}
    % As in the proof of Lemma~\ref{lem:approximate_positive_drift}, we see that $\tilde p_{j+1} \le \tfrac12 \tilde p_{j}$ for $j \ge 2$, 
    where the last step holds for $j\ge 1$ since $\eps n-j \le n-1$. Hence $\tilde p_{\ge 2} \le 2 \tilde p_2 \le \eps^2$.
    
    If no zero-bit is flipped, then the offspring is no improvement. If only a single zero-bit is flipped, then it depends on the function $f$. For $f=\OM$, the offspring is only an improvement in the event $E_{0,1}$ that no one-bit is flipped. Using the bound $q_{0,1} \ge \eps/e$, we thus obtain
    \begin{align}\label{eq:lem:improvement_single_OM_DBV}
        \pimp^{\OM}(\eps n) \le q_{0,1} + \tilde p_{\ge 2} \le q_{0,1} + \eps^2 \le q_{0,1} + e\eps q_{0,1} = (1+e\eps)q_{0,1}.
    \end{align}
    On the other hand, for $f=\DBV$, we still have an improvement in the event $E_{0,1}$. But here we also may have an improvement in the event $E_{1,1}$, depending on which of the two flipped bits has the higher weight. By symmetry, the probability to have an improvement in this case is exactly $1/2$. 
    We also have 
    \begin{align*}
        q_{1, 1} = \binom{\eps n}{1} \frac{1}{n} \binom{(1-\eps)n}{1} \frac{1}{n} \Big(1-\frac{1}{n}\Big)^{n-2} \ge 
        \frac{\eps (1-\eps)}{e} 
    \end{align*}
    by Lemma \ref{lem:basic}. Now using $q_{0,1}\le \eps \le e q_{1,1}/(1-\eps)$, we thus obtain
    \begin{align*}
        \pimp^{\DBV}(\eps n) & \ge q_{0,1} + \tfrac12 q_{1,1} \ge q_{0,1} + \tfrac{1}{2}q_{0,1}(1-\eps)/e \ge q_{0,1}(1+\tfrac{1-\eps}{2e}) \\
        & \stackrel{\eqref{eq:lem:improvement_single_OM_DBV}}{\ge} \pimp^{\OM}(\eps n)\frac{1+\tfrac{1-\eps}{2e}}{1+e\eps},
    \end{align*}
    and the statement follows if $\eps$ is sufficiently small.\qed
    % Any $\onemax$-improvement is a $\dynBV$-improvement\JL{No, that's not true. That is only true if there is only one zero-bit flip.}, which gives
    % \[\pimp^{\OM}(\eps n) \le \ \pimp^{\DBV}(\eps n)\]
    % Now a sufficient condition for a $\dynBV$-improvement which is not a $\onemax$-improvement is the event where all individuals flip exactly one one-bit and one zero-bit and in at least one individual, the zero-bit flip happens in a more significant position than the one-bit flip. This happens wit h
    %
    %Let $E_{i, j}$ denote the event that the offspring $y$ flips $i$ one-bits and $j$ zero-bits, and let $p_{i, j} := \Pr[E_{i,j}]$. The probability that $f^{\DBV}(y) > f^{\DBV}(x)$ given $E_{i, j}$ is $j/(i+j)$, since due to symmetry each flipped bit has the same probability of being the most weighted bit, so that the probability that the most weighted flipped bit is an zero-bit is $j/(i+j)$. It holds that
    %\begin{align*}
    %    p_{imp}^{\DBV} =& \sum_{i=0}^{(1-\eps)n} \sum_{j=1}^{\eps n} p_{i, j} \Pr[f^{\DBV}(y) > f^{\DBV}(x) \mid E_{i, j}] = \sum_{i=0}^{(1-\eps)n} \sum_{j=1}^{\eps n} p_{i, j} \frac{j}{i+j} \\
    %    =& \sum_{j=0}^{(1-\eps)n} p_{0, j} + \sum_{i=1}^{\eps n} \sum_{j=1}^{(1-\eps) n} p_{i, j} \frac{j}{i+j}.
    %\end{align*}
    %Since $p_{i, j} > p_{j, i}$ for $i>j$ when $\eps < 1/2$, namely, when the number of one-bits is larger than the number of zero-bits,
    %\begin{align*}
    %    p_{imp}^{\DBV} =& \sum_{i=0}^{(1-\eps)n} p_{0, j} + \sum_{j=1}^{\eps n} \sum_{i=1}^{j-1} p_{i, j} \frac{j}{i+j} + \sum_{j=1}^{\eps n} \sum_{i=j+1}^{\eps n} p_{i, j} \frac{j}{i+j} + \sum_{j=1}^{\eps n} p_{j, j} \frac{1}{2} \\
    %    >& \sum_{i=0}^{(1-\eps)n} p_{0, j} + \sum_{j=1}^{\eps n} \sum_{i=1}^{j-1} p_{i, j} \frac{j}{i+j} + \sum_{j=1}^{\eps n} \sum_{i=j+1}^{\eps n} p_{j, i} \frac{j}{i+j} \\
    %    =& \sum_{i=0}^{(1-\eps)n} p_{0, j} + \sum_{j=1}^{\eps n} \sum_{i=1}^{j-1} p_{i, j} = p_{imp}^{\OM},
    %\end{align*}
    %where the two nested sums in the second last row corresponds to the parts below and above the diagonal matrix whose entries are $p_{i, j}$. 
    %\qed
\end{proof}


\begin{lemma}
    \label{lem:improvement_population_OM_DBV}
    There exist constants \(\lambda_0 \ge 1\) and \(\beta > 0\) such that the following holds. For all \(\lambda \ge \lambda_0\), there exists \(\varepsilon_0 > 0\) such that for all \(\varepsilon < \varepsilon_0\) we have 
    \begin{align*}
        \qimp^{\DBV}(\eps n, \lambda) \ge (1 + \beta) \qimp^{\OM}(\eps n, \lambda).        
    \end{align*}
    Additionally, \(\varepsilon_0(\lambda) = \Omega( 1 / \lambda )\).
\end{lemma}


\begin{proof}
    Let $0<\alpha<1$ be the constant from Lemma~\ref{lem:improvement_single_OM_DBV}. It is necessary to flip at least one zero-bit to find an improvement, so $\pimp^{\DBV}(\eps n) \le \eps$. By Lemma~\ref{lem:basic} and Lemma~\ref{lem:improvement_single_OM_DBV}, we have
    \begin{align*}
   \qimp^{\DBV}(\eps n, \lambda) & = 1 - (1-\pimp^{\DBV}(\eps n))^\lambda \ge \frac{\pimp^{\DBV}(\eps n)\lambda}{1+\pimp^{\DBV}(\eps n)\lambda} 
   \ge \frac{\tfrac{1}{1-\alpha}\pimp^{\OM}(\eps n)\lambda}{1+\eps\lambda} \\
   & \ge \frac{1-(1-\pimp^{\OM}(\eps n))^{\lambda}}{(1-\alpha)(1+\eps\lambda)} = \frac{\qimp^{\OM}(\eps n, \lambda)}{(1-\alpha)(1+\eps\lambda)}.
    \end{align*}
    Choosing $\eps_0 = \alpha/\lambda$ implies the statement.\qed
    %\begin{align*}
   %\qimp^{\OM}(\eps n, \lambda)=1- (1-\pimp^{\OM}(\eps n))^\lambda \le 1- (1-(1-\alpha)\pimp^{\DBV}(\eps n))^\lambda  \\ \le (1 -\alpha') (1- (1-\pimp^{\DBV}(\eps n))^\lambda) = (1-\alpha') \qimp^{\DBV}(\eps n, \lambda)
%    \end{align*}
%    for $\beta >0$ small enough.\qed
\end{proof}

\begin{lemma}
    \label{lem:improvement_linear_lambda}
    Let \(f \in \{\OM, \DBV\}\). For every \(\gamma > 0\) and \(\lambda \ge 1\) there exists \(\varepsilon_0\) such that for all \(\varepsilon < \varepsilon_0\) we have 
    \begin{align*}
        \qimp^f(\eps n, \lambda) = (1 \pm \gamma)\lambda \pimp^f (\eps n). 
    \end{align*}
    Additionally \(\varepsilon_0( \lambda ) = \Omega(\gamma/\lambda)\).
\end{lemma}

\begin{proof}
    % For both functions, a given child improves the fitness if it flips only a zero-bit. For this reason we must have \(\pimp \ge \varepsilon (1 - 1/n)^{(1 - \varepsilon) n } \ge \varepsilon / e\) by Lemma~\ref{lem:basic}. On the other hand, if the fitness improves then clearly at least a zero-bit must have been flipped meaning that \(\pimp \le \varepsilon\). We thus conclude \(\pimp = \Theta(\varepsilon)\) 
    % For both functions, we have $q_{0, 1} \le \pimp \le 4 q_{0, 1}$, where $q_{0, 1}$ is the probability of flipping 0 one-bit and 1 zero-bit, by a similar argument in Lemma \ref{lem:approximate_positive_drift}. Since $q_{0, 1} = \eps (1-1/n)^{n-1}$, $\pimp = \Theta(\eps)$, we have
    Recall that Lemma~\ref{lem:pimp_roughly_epsilon} guarantees \(\pimp = \Theta(\varepsilon)\). We may express the probability of improvement as
    \begin{align*}
        \qimp = 1-(1-\pimp)^\lambda = 1 - \sum_{i=0}^{\lambda} \binom{\lambda}{i} (- \pimp)^i = \lambda \pimp - \sum_{i=2}^{\lambda} \binom{\lambda}{i} (-1)^i \pimp^i.
    \end{align*}
    If $\lambda=2$, we have $\qimp = (1 - \pimp/2) \lambda \pimp$, choosing $\eps_0$ such that $\pimp/2 < \gamma$ results in $\qimp = (1 \pm \gamma) \lambda \pimp$. For $\lambda > 2$, if we choose $\eps_0$ such that $\pimp < 3/(2(\lambda-2))$, then
    \begin{align*}
        \frac{\binom{\lambda}{i+1} \pimp^{i+1}}{ \binom{\lambda}{i} \pimp^i} = \frac{\lambda-i}{i+1} \pimp < \frac{1}{2},
    \end{align*}
    and 
    \begin{align*}
        \bigg| \sum_{i=2}^{\lambda} \binom{\lambda}{i} (-1)^i \pimp^i \bigg| \le \sum_{i=2}^{\lambda} \binom{\lambda}{i} \pimp^i \le 2 \binom{\lambda}{2} \pimp^2 \le (\lambda \pimp)^2.
    \end{align*}
    Therefore,
    \begin{align*}
        \qimp = \lambda \pimp \pm (\lambda \pimp)^{2} = (1 \pm \lambda \pimp) \lambda \pimp.
    \end{align*}
    By choosing $\eps_0$ such that $\lambda \pimp < \gamma$, we conclude the proof.
    \qed
\end{proof}

We now come to the heart of our proof, which is finding a suitable triple of $\lambda^*$, $s$ and $\eps$.

\begin{lemma}
    \label{lem:construction_equilibrium_OM}
    Let \(f = \OM\). For every \(\xi > 0\) there exists \(\lambda_0 \ge 1\) such that the following holds. For every integer \(\lambda \ge \lambda_0\), there exists \(\tilde{\varepsilon}, \tilde{s}\) depending only on \(\lambda\) such that \(\lambda = \lambda^{*, \OM}(\tilde{\eps} n, \tilde{s})\) and
    \begin{align*}
        \Delta^{\OM}_{\ge 1}(\tilde \eps n, \lambda) = 4 |\Delta^{\OM}_{\le -1}(\tilde \eps n, \lambda)| = (1 \pm \xi)/(\tilde{s} + 1).
    \end{align*}
    \ML{I find it a bit weird that this is the only place where we indicate the dependency in \(\lambda\) with a subscript...}
    Additionally \(\tilde{\varepsilon}(\lambda) = o_{\lambda}( 1/\lambda )\) and \(\tilde{s}(\lambda) = \omega_{\lambda}(1)\).\footnote{The subscript indicates dependency on $\lambda$, i.e., for all $c,C >0$ there exists $\lambda_0$ such that for all $\lambda \ge \lambda_0$ we have $\tilde \eps(\lambda) \le c/\lambda$ and $\tilde s(\lambda) \ge C$.} In particular, for every $\delta, \gamma >0$, if $\lambda_0$ is a sufficiently large constant then $\tilde \eps(\lambda) < \eps_0$ for the $\eps_0$ appearing in Lemmas~~\ref{lem:approximate_negative_drift}, \ref{lem:strong_approximate_negative_drift}, \ref{lem:approximate_positive_drift}, \ref{lem:positive_drift_OM_DBV}, \ref{lem:improvement_single_OM_DBV}, \ref{lem:improvement_population_OM_DBV} and \ref{lem:improvement_linear_lambda}.

\end{lemma}

\begin{proof}
    \ML{I agree with Xun's point and changed a bit the proof. (Btw sorry I didn't get what you meant the first time.) Please have a look.} \XZ{Looks good, thanks! (Sorry for the bad phrasing)}
    Let \(\delta \le \xi\) and \(\gamma, \kappa > 0\) be small constants. We do not yet fix \(\lambda\) but just assume it is large enough so that Lemmas~\ref{lem:approximate_negative_drift}, \ref{lem:strong_approximate_negative_drift} etc. hold simultaneously whenever \(\varepsilon \le \varepsilon_0(\lambda)\), where \(\varepsilon_0\) is taken as the smallest \(\varepsilon_0\) appearing in previous lemmas.

    Since we are considering \(f = \OM\) we have \(p_{\ge 1} = \qimp\); using Lemma~\ref{lem:approximate_positive_drift} followed by Lemma~\ref{lem:improvement_linear_lambda} we find
    \begin{align*}
        \Delta_{\ge 1} = (1 \pm \delta) p_{\ge 1} = (1 \pm \delta) \qimp = (1 \pm \delta)(1 \pm \gamma) \pimp \lambda.
    \end{align*}
    Now using Lemma~\ref{lem:strong_approximate_negative_drift} we may estimate the negative contribution as 
    \begin{align*}
        \Delta_{\le -1} = -(1 \pm \delta) (1 - e^{-1})^\lambda.
    \end{align*}
    
    % to estimate the negative contribution \(\Delta_{\le -1}\), we see that the drift of \(Z\) at \(\varepsilon n, \lambda\) is 
    % \begin{align*}
    %     (1 \pm \delta)(1 \pm \gamma) \pimp \lambda - (1 \pm \delta)(1 - e^{-1})^\lambda. \numberthis \label{eq:lem:construction_equilibrium_OM_1}
    % \end{align*}
    
    Recall now that \(\pimp\) is the probability that a single child flips more zero-bits than one-bits and is of order \(\Theta(\varepsilon)\). 
    Hence when \(\varepsilon = \varepsilon_0(\lambda)\), every \(\lambda\) large enough is such that all the above holds and such that \(\Delta_{\ge 1} \) is much bigger than \(|\Delta_{\le -1}|\).
    %Hence when \(\varepsilon = \varepsilon_0(\lambda)\), every \(\lambda\) large enough is such that all the above holds and such that the positive term of \eqref{eq:lem:construction_equilibrium_OM_1} is at least four times the (absolute value) \XZ{why not just write $|\Delta_{\le -1}|$? and why do we have \eqref{eq:lem:construction_equilibrium_OM_1}?}. \ML{The drift is at least \(\Delta_1 + \Delta_{\le -1}\). The first term is given in the display \(\Delta_1 = (1 \pm \delta) \pimp \lambda \) and the second term is given by Lemma~\ref{lem:strong_approximate_negative_drift} \(\Delta_{\ge -1} = - (1 \pm \delta)(1 - e^{-1})^\lambda\). And this gives \eqref{eq:lem:construction_equilibrium_OM_1}.} \XZ{Yes, I got that. I meant we just want to have $\Delta_{\ge 1} = 4 |\Delta_{\le -1}|$ for the lemma, and the drift does not seem to be relevant here, so why we have an expression for it?}
    For this fixed \(\lambda\) we then make \(\varepsilon\) continuously vary from \(\varepsilon_0(\lambda)\) to \(0\). The negative term does not change much while the positive one continuously drops to \(0\). Hence there must exist some \(\varepsilon\) at which the ratio is exactly \(4\) and one easily checks that this happens for some \(\varepsilon = \Theta( (1 - e^{-1})^\lambda / \lambda ) = o(1 / \lambda)\).
    
    We set \(\tilde{\varepsilon}\) to be exactly this \(\varepsilon\). We then define \(\tilde s\) so that \( 1/(\tilde s + 1) = \qimp\). Since \(\Delta_{\ge 1} = (1 \pm \delta)\qimp \) the equality is proved. All that remains is to check that \(\tilde{s}\) has the correct order: this comes from \(\tilde s = \Theta( 1/(\lambda \tilde \varepsilon) ) = \omega_{\lambda}(1)\) using Lemma~\ref{lem:improvement_linear_lambda}, which concludes the proof.\qed
\end{proof}

Naturally, the lemma above implies that for parameters \(\lambda, \tilde s\) and at distance \(\tilde{\varepsilon} n\) from the optimum, the drift of \(Z\) for \OM is roughly \(\Delta^{\OM} = \Delta^\OM_{\ge 1} + \Delta^\OM_{\le -1} = \frac34 \Delta^{\OM}_{\ge 1} > 0\).
For this triple, we can show that $\lambda^{*,\DBV}$ is much smaller than $\lambda = \lambda^{*,\OM}$. %\XZ{was this $\approx$ due to a previous version? In the proof we just have the equality}.
This smaller $\lambda^*$ will be the reason why the drift of $Z$ is negative for \DBV.
%, even though the triple was chosen such that the drift of $Z$ is positive for \onemax. 
\XZ{Again I find it confusing to talk about positive/negative drift for $Z$} \ML{Reformulated a bit the sentence above. Is it better with the current version of the proof?} \XZ{Looks great!}

\begin{corollary}
    \label{cor:equilibrium_OM_DBV}
    There exists \(\kappa > 0\) and \(\lambda_0 \ge 1\) such that the following holds. Let \(\lambda \ge \lambda_0\) and $\tilde s = \tilde s(\lambda)$, $\tilde \eps = \tilde \eps(\lambda)$ as in Lemma~\ref{lem:construction_equilibrium_OM}. Then  
    \begin{align}\label{eq:cor:equilibrium_OM_DBV}
        \lambda^{*, \DBV}(\tilde{\varepsilon} n, \tilde{s} ) \le (1 - \kappa) \lambda.
    \end{align}
    We also have \(\lambda^{*, \OM}(\tilde \varepsilon n, \tilde{s}) = \Omega(\lambda)\); in particular for \(\lambda\) large enough, Lemmas~~\ref{lem:approximate_negative_drift}, \ref{lem:strong_approximate_negative_drift}, \ref{lem:approximate_positive_drift}, \ref{lem:positive_drift_OM_DBV}, \ref{lem:improvement_single_OM_DBV}, \ref{lem:improvement_population_OM_DBV} and \ref{lem:improvement_linear_lambda} also hold for \(\lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s)\).
\end{corollary}

\begin{proof}
    Recall that Lemma \ref{lem:construction_equilibrium_OM} guarantees that $\lambda^{*,\OM}(\tilde \eps n,\tilde s) = \lambda$. 
    % Hence, it suffices to prove~\eqref{eq:cor:equilibrium_OM_DBV} with 
    % $\lambda^{*,\OM}(\tilde s,\tilde \eps)$ instead of $\lambda$. 
    Moreover, it also guarantees that for $\lambda_0$ large enough we can achieve $\tilde \eps \le \eps_0$ for the $\eps_0$ from Lemma~\ref{lem:improvement_single_OM_DBV}. We compare the two different $\lambda^{*,f}$ by plugging in their definition from~\eqref{eq:def:lambdastar},
    \begin{align}\label{eq:cor:equilibrium_OM_DBV2}
        \frac{\lambda^{*, \DBV}(\tilde \eps n, \tilde s)}{\lambda^{*, \OM}(\tilde \eps n, \tilde s)} = \frac{\log_{(1 - \pimp^{\DBV}(\tilde \eps n))}\big(\tfrac{s}{1+s}\big)}{\log_{(1 - \pimp^{\OM}(\tilde \eps n ))}\big(\tfrac{s}{1+s}\big)} = \frac{-\log(1-\pimp^{\OM}(\tilde \eps n))}{-\log(1-\pimp^{\DBV}(\tilde \eps n))},
    \end{align}
    where the minus signs are introduced for clarity, so that numerator and denomi\-na\-tor are positive.
    From Lemma~\ref{lem:improvement_single_OM_DBV}, we know that there exists $\alpha >0$ such that $\pimp^{\OM}(\tilde \eps n) \le ( 1 - \alpha ) \pimp^{\DBV}(\tilde \eps n)$. Hence, the right hand side of~\eqref{eq:cor:equilibrium_OM_DBV2} is at most $\sup_{z\in (0,1)}L(z)$ for $L(z) := \log(1-(1-\alpha)z)/\log(1-z)$. The function $L$ is continuous and satisfies $L(z) < 1$ in $(0,1)$, since $-\log(1-(1-\alpha)z) < -\log(1-z)$. Moreover, it satisfies $L(z) \to 0$ as $z\to 1$ and $L(z) \to 1-\alpha$ as $z\to 0$. Hence, the supremum is either $(1-\alpha)$ or it is a maximum taken at some intermediate point. In any case, it is strictly smaller than one. This proves that~\eqref{eq:cor:equilibrium_OM_DBV2} is at most $1-\kappa$ for some $\kappa >0$.
    
    We now turn to the second statement. First of all we choose a small \(\gamma > 0\) and assume that \(\lambda\) was chosen large enough so that Lemma~\ref{lem:improvement_linear_lambda} holds for this \(\gamma\). 
    % From Lemma~\ref{lem:construction_equilibrium_OM}, \(\lambda^{*, \OM}(\tilde \varepsilon n, \tilde s) \ge \lambda + 1\) so Lemma~\ref{lem:improvement_population_OM_DBV} also applies to\footnote{To be precise, we may need to take \(\lambda\) slightly larger to compensate for the additional \(+1\). This works because \(\lambda, \lambda^{*, OM}\) behave similarly asymptotically, Lemma~\ref{lem:improvement_population_OM_DBV} requires \(\varepsilon = O(1/\lambda)\) and Lemma~\ref{lem:construction_equilibrium_OM} gives \(\varepsilon = o(1 / \lambda)\).} \(\lambda^{*, \OM}(\tilde \varepsilon n, \tilde s)\).
    We just proved that \(\lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s) \le \lambda\) so Lemma~\ref{lem:improvement_linear_lambda} must also hold for this \(\lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s)\). In particular, we have 
    \begin{align*}
        \begin{cases}
            \qimp^{\OM}( \tilde{\varepsilon} n, \lambda^{*, \OM}(\tilde \varepsilon n, \tilde s) ) = (1 \pm \gamma) \pimp^{\OM}(\tilde \varepsilon n) \lambda^{*, \OM}(\tilde \varepsilon n, \tilde s); \\
            \qimp^{\DBV}( \tilde{\varepsilon} n, \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s) ) = (1 \pm \gamma) \pimp^{\DBV}(\tilde \varepsilon n) \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s).
        \end{cases}
    \end{align*}
    By definition, we have \(\qimp^{\DBV}( \tilde{\varepsilon} n, \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s) ) = \qimp^{\OM}( \tilde{\varepsilon} n, \lambda^{*, \OM}(\tilde \varepsilon n, \tilde s) ) = 1/(\tilde s + 1)\), meaning that 
    \begin{align*}
         (1 \pm \gamma) \pimp^{\OM}(\tilde \varepsilon n) \lambda^{*, \OM}(\tilde \varepsilon n, \tilde s)
          &=  (1 \pm \gamma) \pimp^{\DBV}(\tilde \varepsilon n) \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s).
    \end{align*}
    Recall that
    \(\pimp^{\OM}(\tilde{\varepsilon}n), \pimp^{\DBV}(\tilde{\varepsilon} n)\) are the probabilities that a single child improves the fitness for \OM resp.\ \DBV and are both of order \(\Theta(\tilde \varepsilon)\) by Lemma~\ref{lem:pimp_roughly_epsilon}. Hence, they may only differ by a constant multiplicative factor and the same must be true for $\lambda^{*, \OM}(\tilde \varepsilon n, \tilde s)$ and \(\lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s)\). This finishes the proof.
    \qed
\end{proof}


\begin{lemma}
    \label{lem:construction_inefficient_DBV}
    Let \(f = \DBV\). There exists \(\lambda_0 \ge 1\) such that for all \(\lambda \ge \lambda_0\) there are \(\nu,\eps' > 0\) such that the following holds. Let \(\tilde s = \tilde{s}(\lambda), \tilde \varepsilon = \tilde{\varepsilon}(\lambda)\) as in Lemma~\ref{lem:construction_equilibrium_OM}. If \(Z^t = (\tilde \varepsilon \pm \varepsilon') n\) and \(\lambda^t \le \lambda^{*,\DBV}(Z^t, \tilde{s}) + 1\) we have 
    \begin{align*}
        \EE[Z^t - Z^{t+1} \mid x^t, \lambda^t] \le -\nu.
    \end{align*}
\end{lemma}
\begin{proof}
    We fix $\delta >0$ to be chosen later and choose \(\lambda\) sufficiently large so that Lemmas~\ref{lem:approximate_negative_drift}, \ref{lem:strong_approximate_negative_drift}, \ref{lem:strong_approximate_negative_drift}, \ref{lem:approximate_positive_drift}, \ref{lem:positive_drift_OM_DBV}, \ref{lem:lambda_changes_slowly} and Corollary~\ref{cor:equilibrium_OM_DBV} hold for \(\lambda^{*, \DBV}(\tilde \varepsilon n , \tilde s)\). Note that this is possible by Corollary~\ref{cor:equilibrium_OM_DBV}, which guarantees that \(\lambda^{*,\DBV}(\tilde \varepsilon n, \tilde s)\) can be arbitrarily large as long as \(\lambda\) is.
    
    Lemma~\ref{lem:lambda_changes_slowly} guarantees the existence of an \(\varepsilon'\) (which may and does depend on \(\lambda\)) such that for all \(Z = (\tilde \varepsilon \pm \varepsilon')n\) we have \(\lambda^{*, \DBV}(Z, \tilde s) = \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde s) \pm 1\). To prove the statement, it is then sufficient to prove it for all \(Z^t = (\tilde \varepsilon \pm \varepsilon')n \) and \(\lambda^t \le \lambda^{*, \DBV}(\tilde \eps n, \tilde s) + 2\).

    For any such \(\lambda^t\), the drift of \(Z\) for \(\DBV\) is 
    \begin{align*}
        \Delta^{\DBV}_{\ge 1}(Z^t, \lambda^t) + \Delta^{\DBV}_{\le -1}(Z^t, \lambda^t).
    \end{align*}
    From Lemma \ref{lem:comparison_positive_drift_OM_DBV} we know that this drift is at most 
    \begin{align*}
        \Delta^{\OM}_{\ge 1}(Z^t, \lambda^t) + \Delta^{\OM}_{\le -1}(Z^t, \lambda^t).
    \end{align*}
    By Lemma~\ref{lem:approximate_positive_drift} the positive contribution of this drift is at most \((1 + \delta) \Delta^{\OM}_1(Z^t, \lambda^t) \le (1 + \delta) \qimp^{\OM}(Z^t, \lambda^t)\). By Corollary~\ref{cor:equilibrium_OM_DBV} we know that \(\lambda^t \le \lambda^{*, \DBV}(\tilde{\varepsilon}n, \tilde{s}) + 2 \le \lambda^{*, \OM}(\tilde{\varepsilon}n, \tilde{s})\), which implies that \(\qimp^{\OM}(Z^t, \lambda^t) \le  1/(\tilde s+1)\).
    
     Lemma~\ref{lem:strong_approximate_negative_drift} guarantees that \(\Delta^{\OM}_{\le -1}\) is exponential in \(\lambda\), while Corollary~\ref{cor:equilibrium_OM_DBV} states that \(\lambda^{*, \DBV}(\tilde \varepsilon n, \tilde{s}) \le (1 - \kappa) \lambda\). Combining both, we obtain 
    \begin{align*}
         | \Delta_{\le -1}^{\OM}(Z, \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde{s}) + 2) |
            &\ge (1 \pm \delta) (1 - e^{-1})^{(1-\kappa) \lambda + 2}.
    \end{align*}
    By Lemma~\ref{lem:construction_equilibrium_OM}, we have \(|\Delta_{\le -1}^{\OM}( \tilde \varepsilon n, \lambda)| = (1 \pm \delta) \frac{1}{4(\tilde s+1)}\), and a new application of Lemma~\ref{lem:strong_approximate_negative_drift} gives that \((1 \pm \delta) / (4(\tilde s+1)) = (1 \pm \delta) (1 - e^{-1})^\lambda \). Replacing in the display above gives 
    \begin{align*}
         |\Delta_{\le -1}^{\OM}(Z, \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde{s}) + 2) |
            &\ge (1 \pm 3\delta) (1 - e^{-1})^{-\kappa \lambda + 2} \frac{1}{4(\tilde s+1)} \ge \frac{2}{\tilde s+1},
    \end{align*}
    as \(\lambda\) may be chosen large enough compared to \(\kappa, \delta\).
    
    % as long as \(\lambda\) is large enough. Here the first equality is obtained using Corollary~\ref{cor:equilibrium_OM_DBV}.
    Since \(\lambda^t \le \lambda^{*, \DBV}(\tilde \varepsilon n, \tilde{s}) + 2 \) the negative contribution to the drift may only be worse. In the range of \(Z^t, \lambda^t\) from the lemma, we see that 
    \begin{align*}
        \EE[ Z^t - Z^{t+1} \mid x^t, \lambda^t ]
            &\le (1 + \delta) \frac{1}{\tilde s+1} - \frac{2}{\tilde s+1}
            \le -\frac{1}{2(\tilde s+1)},
    \end{align*}
    which concludes the proof.\qed
\end{proof}

We could easily see that the drift for \onemax at the parameter triple defined in Lemma~\ref{lem:construction_equilibrium_OM} is positive. Moreover, we want to show that the \saolea can not only pass this point, but continues all the way to the optimum. To this end, we define a more general potential function already used in~\cite{hevia2021arxiv} and~\cite{kaufmann2022arxiv}.


\begin{definition}
    We define 
    \begin{align*}
        h(\lambda) := -K \log_F \lambda,
    \end{align*}
    with \(K = 1/2\). We also define
    \begin{align*}
        g(x, \lambda) := \ZM(x) + h(\lambda).
    \end{align*}
\end{definition}

For convenience we will write \(Z^t = \ZM(x^t)\), \(H^t = h(\lambda^t)\) and \(G^t = Z^t + H^t = g(x^t, \lambda^t)\).

\begin{lemma}
    \label{lem:drift_H}
    Let \(f = \OM\). At all times \(t\) we have 
    \begin{align*}
        \EE \left[ H^t - H^{t+1} \mid x^t , \lambda^t \right] = \tfrac{K}{s}(1- (s+1)\qimp(x^t,\round{\lambda^t})).
    \end{align*}
\end{lemma}

\begin{proof}
    We have $H^{t+1} = -K\log_F(\lambda^t/F) = H^t+K$ in case of an improvement, and $H^{t+1} = H^t-K/s$ otherwise. Hence, the drift of $H^t$ is
\begin{align*}
    \EE[H^t-H^{t+1} \mid x^t,\lambda^t] = -K\qimp + (1-\qimp)\tfrac{K}{s} = \tfrac{K}{s}(1- (s+1)\qimp).\qquad \qed
\end{align*}
%    \qed
\end{proof}

With these choices, the drift of $G^t$ is positive for \emph{all} $\eps \le \tilde \eps$ and $\lambda^t \ge \lambda-1$.


\begin{corollary}
    \label{cor:OM_positive_drift}
    Let $f=\OM$. There exists \(\lambda_0 \ge 1\) such that the following holds for all \(\lambda \ge \lambda_0\). Let $s = \tilde s = \tilde s(\lambda)$, $\eps = \tilde \eps = \tilde \eps(\lambda)$ be as in Lemma~\ref{lem:construction_equilibrium_OM}. There exist \(\rho(\lambda), \eps'(\lambda)\) such that if \(1 \le  Z^t \le (\varepsilon +\eps')n\) and \(\lambda^t \ge \lambda-1\), then 
    \begin{align*}
        \EE [ G^t - G^{t+1} \mid Z^t, \lambda^t ] \ge \rho.
    \end{align*}
\end{corollary}

\begin{proof}
    \ML{I think I agree with Xun and there were leftovers of previous proofs. I cleaned a bit and it looks good to me, but maybe someone can check that I didn't remove something needed for the proof.}
    \XZ{Looks good to me}
    Let \(\xi = \delta = \gamma = \kappa > 0\) be sufficiently small constants and let \(\lambda_0\) be sufficiently large so that Lemmas~\ref{lem:strong_approximate_negative_drift}, %\ref{lem:improvement_linear_lambda}, 
    \ref{lem:construction_equilibrium_OM} hold. 
    %Let \(\varepsilon = \tilde{\varepsilon}(\lambda), s = \tilde{s}(\lambda)\) be as in Lemma~\ref{lem:construction_equilibrium_OM} so that we have $\lambda^{*, \OM}(\eps n, s) = \lambda$. 
    By Lemma~\ref{lem:lambda_changes_slowly}, there exists a small \(\varepsilon' > 0\) such that \(\lambda^{*, \OM}((\varepsilon + \varepsilon')n, s) \ge \lambda - 1/2\).
    %In particular, the hypothesis \(\lambda^t \ge \lambda - 1\) guarantees that we also have \(\lambda^t \ge \lambda^{*, \OM}( Z^t, s ) - 1\) \XZ{This holds if $\lambda > \lambda^{*, \OM}(Z^t, s)$, but $Z^t$ can be rather small in this lemma. Were the last two sentence from a previous version? The $\lambda^*$s do not appear later in the proof}. Additionally, since the \(\tilde{\varepsilon}\) provided by Lemma~\ref{lem:construction_equilibrium_OM} decreases very fast with \(\lambda\), we can guarantee that if \(\lambda_0\) is chosen large enough and \(\varepsilon'\) small enough, then all precedent lemmas hold for this \(\lambda\) and \(\varepsilon + \varepsilon'\).
    
    We seek to estimate the drift of \(G\) when \(Z^t \le (\varepsilon + \varepsilon') n\) and \(\lambda^t \ge \lambda - 1\). Using Lemma~\ref{lem:drift_H}, we see that this drift is  
    \begin{align*}
        \EE[ G^t - G^{t+1} \mid Z^t, \lambda^t ]
            &= \Delta_{\ge 1}(Z^t, \lambda^t) + \Delta_{\le -1}(Z^t, \lambda^t) \\
                &\qquad \qquad \qquad - K\qimp(Z^t, \lambda^t) + K (1 - \qimp(Z^t, \lambda^t)) / s.
    \end{align*}
    
    From Lemma~\ref{lem:strong_approximate_negative_drift} applied for both \(Z^t\) and \(\tilde\varepsilon n\) and from Lemma~\ref{lem:construction_equilibrium_OM} we know that
    \begin{align*}
            |\Delta_{\le -1}(Z^t, \lambda)| 
                &= (1 \pm \delta) (1 - e^{-1})^{\lambda} = (1 \pm \delta)^2|\Delta_{\le -1}(\varepsilon n, \lambda)| \\
                &=  (1 \pm \delta)^3/(4(s+1)). 
    \end{align*}
    
    Applying Lemma~\ref{lem:strong_approximate_negative_drift}, now for \(\lambda-1\), we have \(\Delta_{\le -1}(Z^t, \lambda - 1) = (1 \pm \delta) (1 - e^{-1})^{\lambda - 1} \), which by the above must be at most 
    \begin{align*}
        |\Delta_{\le -1}(Z^t, \lambda - 1)| \le (1 \pm \delta)^5 \frac{1}{4(1 - e^{-1})(s+1)} \le \frac{1}{2(s+1)}.
    \end{align*}
    As \(\Delta_{\le -1}(Z^t, \cdot )\) is decreasing, this same bound must hold whenever \(\lambda^t \ge \lambda - 1\). We also observe that since we are considering \(\OM\), we have \(\Delta_{\ge 1} \ge \qimp\).
    
    Now replacing in the expression of the drift with \(K = 1/2\), the drift is at least
    \begin{align*}
        \EE[ G^t - G^{t+1} \mid Z^t, \lambda^t ]
            &\ge \qimp - \frac{1}{2(s+1)} - \frac{\qimp}{2} + \frac{1}{2s} - \frac{\qimp}{2s} \\
            &= \frac{1}{2 s(s+1)} + \frac{\qimp}{2}(1 - 1/s) \\
            &\ge \frac{1}{2s(s+1)},
    \end{align*}
    since for a choice of \(\lambda_0\) large enough we may assume that \(s > 1\) by Lemma~\ref{lem:construction_equilibrium_OM}. Setting \(\rho(\lambda) = 1 / (2 s (s+1))\) concludes the proof.
    \qed
\end{proof}

% \begin{comment}


% \todo{I need this extra lemma. I add it here with proof but it probably should have its place above.}

% \begin{lemma}
%     \label{lem:lambda_changes_slowly}
%     Let \(f \in \{\OM, \DBV\}\). For all \(\varepsilon, s,\rho > 0\) there exists \(\delta\) such that 
%     \begin{align*}
%         \lambda^{*, f}((\varepsilon - \delta)n, s) - \lambda^{*, f}((\varepsilon + \delta)n, s) \le \rho.
%     \end{align*}
% \end{lemma}
% \begin{proof}
%     This is a simple consequence of the definition: 
%     \begin{align*}
%         \lambda^{*,f}(Z, s) = \log_{1 - \pimp(Z)}(s/s+1) = \frac{\log(s/s+1)}{\log(1 - \pimp(Z))}.
%     \end{align*}
%     If \(Z = \varepsilon n\) then \(\pimp(Z) = \Theta(Z/n)\) and increasing or decreasing it by \(\delta n\) for a small \(\delta\) changes \(\pimp\) only by a small constant. Choosing \(\delta\) sufficiently small enough, we can guarantee that this difference is at most \(\rho/2\) in both directions, that is at most \(\rho\) in total.\qed
% \end{proof}

% \end{comment}

Now we are ready to formulate and prove the main result of this paper.

\begin{theorem}
    \label{thm:existence_threshold}
    Let $F=1+\eta$ for some $\eta = \omega(\log n/n) \cap o(1/\log n)$. There exist constants \(s, \varepsilon\) such that with high probability the \saolea with success ratio $s$, update strength $F$ and mutation rate $1/n$ starting with $Z^0 =\eps n$,
    \begin{enumerate}[a)]
        \item finds the optimum of \onemax in $O(n)$ generations;
        \item does not find the optimum of \dynBV in a polynomial number of generations.
        \end{enumerate}
\end{theorem}

\begin{proof}
    Let $\delta=\gamma = 1/10$ \XZ{does not seem to appear in the proof}, and choose \(\lambda\) so large that Lemmas~\ref{lem:approximate_negative_drift}, \ref{lem:strong_approximate_negative_drift}, \ref{lem:approximate_positive_drift}, \ref{lem:positive_drift_OM_DBV}, \ref{lem:improvement_single_OM_DBV}, \ref{lem:improvement_population_OM_DBV} and \ref{lem:improvement_linear_lambda} are satisfied. Let \(s := \tilde{s}(\lambda)\) and \(\varepsilon = \tilde{\varepsilon}(\lambda)\) as in Lemma~\ref{lem:construction_equilibrium_OM} so that Corollary~\ref{cor:equilibrium_OM_DBV} and Lemma~\ref{lem:construction_inefficient_DBV} hold.
    
    We first prove a). Set $f:=\onemax$, and let $\eps' = \eps'(\lambda)$ be small enough to apply Corollary~\ref{cor:OM_positive_drift}. 
    We will first argue that $\lambda^t$ quickly reaches a value of at least $\lambda - 7/8$ and stays above $\lambda - 1$ afterwards. Note that by definition of $\tilde \eps$, we have $\qimp(\tilde \eps n,\lambda) = 1/(s+1)$, and hence
    \begin{align*}
        \qimp(\tilde \eps n,\lambda - 1/4) < \qimp(\tilde \eps n,\lambda) = \tfrac{1}{s+1}.
    \end{align*}
    Up to potentially reducing \(\varepsilon'\), we may apply Lemma~\ref{lem:lambda_changes_slowly} and get
    %, there exists $\eps' >0$ \XZ{conflicting with the one defined before} such that
    \begin{align*}
        \qimp((\tilde \eps+\eps') n,\lambda-1/4) = \tfrac{1}{s+1},
    \end{align*}
    or in other words $\lambda^*((\tilde \eps+\eps')n, s)= \lambda - 1/4$. Therefore, $\round{\lambda - 7/8} \le \lambda - 3/8 < \lambda^*((\tilde \eps+\eps')n, s)$, and by Lemma~\ref{lem:drift_H} we have for all $1<Z^t \le (\tilde \eps + \eps')n$ and all $\lambda^t \le \lambda - 7/8$,
    \begin{align*}
        E[H^t-H^{t+1} \mid Z^t,\lambda^t] & =   \tfrac{K}{s}(1-(s+1)\qimp(Z^t,\round{\lambda^t})) \\
        & \ge  \tfrac{K}{s}(1-(s+1)\qimp((\tilde\eps+\eps')n,\lambda - 3/8)) \ge d, 
    \end{align*}
    for a suitable constant $d>0$. Therefore, $H^t$ has positive drift as long as $1<Z^t \le (\tilde \eps + \eps')n$ and $\lambda^t \le \lambda - 7/8$. By Lemma~\ref{lem:small-steps}, we may assume that $Z^t$ changes by at most $\log n$ in all of the first $\eps'n/(2\log n)$ steps. In particular, we have $Z^t \le (\tilde\eps +\eps'/2)n$ during this time. Hence, $H^t$ has constant positive drift until either $\eps'n/(2\log n)$ steps are over or until it hits $-K\log_F(\lambda-7/8)$. Since $H^0 = -K\log_F(1) = 0$, by the additive drift theorem, the latter option happens after at most $\tfrac{K}{d}\log_F (\lambda - 7/8) = O(1/ \log F) = O(1/\eta)$ steps in expectation. Moreover, the same holds with high probability after at most $2\tfrac{K}{d}\log_F (\lambda-7/8) = O(1/\eta)$ steps by concentration of hitting times for additive drift, Theorem~\ref{thm:AdditiveDrift}, since $H$ changes by definition by at most one in each step. Since $1/\eta = o(n/\log n)$, with high probability, $\lambda^t \ge \lambda - 7/8$ happens before $Z^t$ reaches $(\tilde \eps+\eps'/2)n$. Let us call the first such point in time $t_0$.
    
    Now we show that after time $t_0$, the population size $\lambda^t$ stays above $\lambda - 1$. Let $T > t_0$ denote the first point in time after $t_0$ when either $Z^t \ge (\tilde \eps + \eps')n$ or when $\lambda^t \le \lambda - 1$. We have already established that $H^t$ has at least constant positive drift for $t \in [t_0,T]$ \XZ{is not it only true for $\lambda^t \le \lambda - 7/8$?}. In order for $\lambda$ to decrease from $\lambda-7/8$ to $\lambda-1$ the potential must increase by $K\log_F(\lambda - 7/8) - K\log_F(\lambda - 1) = \Omega(1/\log F) = \Omega(1/\eta) = \omega(\log n)$. By the negative drift theorem, Theorem~\ref{thm:NegativeDrift}, with high probability this does not happen within $O(n^2)$ steps. 
    
    On the other hand, since we may assume by Lemma~\ref{lem:small-steps} that $\lambda^t \le n^2$ for a superpolynomial number of steps, we have $0 \le Z^t- G^t \le \log_F(n^2) = O(\tfrac1\eta\log n) = o(n)$. In particular, the event $Z^t > (\tilde \eps + \eps')n$ implies $G^t > (\tilde \eps + \tfrac34\eps')n \ge Z^{t_0} + \eps' n/4 \ge G^{t_0} + \eps' n/4$. In other words, $Z^t$ can only exceed $(\tilde \eps + \eps')n$ if the potential $G^t$ increases by at least $\eps'n/4$. We will show in the following that this is unlikely.
    
     By Corollary~\ref{cor:OM_positive_drift} the potential $G^t = Z^t+H^t$ has constant drift towards zero while $1<Z^t \le  (\tilde \eps + \eps')n$ and $\lambda^t \ge \lambda-1$. Moreover, we may assume that $Z^t$ changes by at most $\log n$ in each step by Lemma~\ref{lem:small-steps}, and $H^t$ changes by at most one in each step. Therefore, by the negative drift theorem with scaling, Theorem~\ref{thm:NegativeDrift}, with high probability $G^t$ does not increase by $\eps' n/4$ within $n^2$ steps. 
    
    We have established that with high probability, for $n^2$ steps none of the events $\lambda^t < \lambda - 1$ and $Z^t > (\tilde \eps + \eps')n$ happens. Hence, by Corollary~\ref{cor:OM_positive_drift} the potential $G^t$ has a positive drift for $n^2$ steps, or until $Z^t$ hits zero. Since we start with a potential of at most $Z^{t_0} + H^{t_0} \le Z^{t_0} = O(n)$, with high probability the event $Z^t =0$ happens within $O(n)$ steps by the tail bounds on hitting times for additive drift, Theorem~\ref{thm:AdditiveDrift}. This proves a).  
    
    For b), we set $f:= \DBV$, and we will work directly with the potential $Z^t$ instead of $G^t$. Let $\eps' >0$ be the constant from Lemma~\ref{lem:construction_inefficient_DBV}. We first show that as long as $Z^t \ge (\tilde\eps-\eps')n$, for a superpolynomial number of steps we have $\lambda^t \le \lambda^{*,\DBV}(\tilde s, \tilde \eps) + 1$ 
    \XZ{want $\lambda^t \le \lambda^{*, \DBV}(Z^t, \tilde s)$ from the lemma}
    so that we may apply Lemma~\ref{lem:construction_inefficient_DBV}. As for case a), by decreasing $\eps'$, 
    we can achieve that for all \(\lambda^t \ge \lambda^{*, \DBV}(\tilde{s}, \tilde \eps + \eps') + 3/4\) and all \(Z^t = (\tilde \eps \pm \eps')n\),
    %we can achieve that for all $\lambda^t+3/4 \le \lambda^{*,\DBV}(\tilde s, \tilde \eps) +1$ and all $Z^t \ge (\tilde \eps -\eps')n$,
    \begin{align*}
        % \qimp(Z^t,\lfloor\lambda^t\rceil) \ge \qimp((\tilde \eps +\eps') n, \lambda^{*,\DBV}(\tilde s, \tilde \eps) +1/4) > \tfrac{1}{s+1},
        \qimp(Z^t,\lfloor\lambda^t\rceil) \ge \qimp((\tilde \eps +\eps') n, \lambda^{*,\DBV}(\tilde s, \tilde \eps + \eps') + 1/8) > \tfrac{1}{s+1},
    \end{align*}
    \XZ{Here we need a negative drift as compared to a) since we would like $\lambda^t$ to be bounded. So we would like to have something like the inequality above, but the first sign there is wrong.
        \begin{align*}
        % \qimp(Z^t,\lfloor\lambda^t\rceil) \ge \qimp((\tilde \eps +\eps') n, \lambda^{*,\DBV}(\tilde s, \tilde \eps) +1/4) > \tfrac{1}{s+1},
        \qimp(Z^t,\lfloor\lambda^t\rceil) \ge \qimp(Z^t, \lambda^{*,\DBV}(Z^t, \tilde s) + 1/4) > \tfrac{1}{s+1},
    \end{align*}
    }
    which implies a constant positive drift of $H^t$  As in case a), with high probability $\lambda^t$ does not exceed $\lambda+1$ for a superpolynomial number of steps, as long as $Z^t \ge (\tilde \eps -\eps')n$ is satisfied. On the other hand, as long as $\lambda^t \le \lambda^{*,\DBV}(\tilde s, \tilde \eps)+1$, $Z^t$ has constant drift away from the optimum in the interval $(\tilde \eps \pm \eps')n$. By the negative drift theorem with scaling, with high probability $Z^t$ stays above $(\tilde \eps -\eps')n$ for a superpolynomial number of steps. This concludes the proof of b).\qed
\end{proof}
\XZ{For he notation, we want to use $s$ and $\eps$ instead of $\tilde s$ and $\tilde \eps$ in Corollary \ref{cor:OM_positive_drift} and Theorem~\ref{thm:existence_threshold}, right?}
% \XZ{does this look correct to you in the first inequality? It is probably $(\tilde \eps - \eps')$, but why $\qimp$ decreases with more offspring?}. \ML{I slightly changed the formulation, but I think it is ok. Essentially we are saying that we can choose \(\eps'\) super small so that the difference between the \(\lambda^*(\tilde{\eps} \pm \eps')\) is very small. So if \(\lambda^t\) is a constant above \(\lambda^*(\tilde{\eps})\), it is also a constant (a bit smaller) above all the \(\lambda^*\). And because of this, the drift of \(H\) is positive.}


% \begin{theorem}\label{thm:negative}
%     negative result.
% \end{theorem}

% \begin{proof}
% Drift is negative for $\lambda = \lambda^*$. Show that small fluctuations of $(1\pm \gamma)\lambda$ change the drift around $\lambda^*$ by at most factors $1\pm O(\gamma)$. We can always assume that $s$ small enough, $\lambda^*$ large enough, $\eps$ small enough (need to add these conditions to the lemmas of the drift statement then). Similarly if $Z^t$ fluctuates in $(1\pm o(1))\eps n$.

% Show that whp we have never $\lambda > n^{10}$.

% Whenever $Z^t$ enters region around $\eps n$ with $\lambda \le n^{10}$, it quickly (time $O((\log n)/(F-1))$) goes down to $(1\pm o(1))$ because it has drift. In this time it can't make more progress than $O(\text{time} \cdot\log n)$, which is negligible. Afterwards, $Z^t$ has negative drift and leaves region again. All with high probability, even over superpolynomial trials.
% \end{proof}

% \begin{proposition}\label{prop:drift_stays_positive}
% Let $s,\eps >0$ be as in Proposition~\ref{prop:drift}. Then for all $Z^t \le \eps n$, we have positive drift for \onemax for $\lambda = \lambda^*(Z^t,s)$,
% \begin{align*}
%     \Delta^t_{\OM}(Z^t,\lambda^*(Z^t,s)) \ge c s_0.
% \end{align*}    
% \end{proposition}
% \begin{proof}
% We use the decomposition 
% \begin{align*}
%     \Delta = p_1 + \Delta_{\ge 2} + \Delta_{\le -1}.
% \end{align*}
% By Proposition~\ref{prop:drift}, for $Z^t = \eps n$ and $\lambda = \lambda^*(s,\eps)$ we have $p_1 + \Delta_{\le -1} \ge c s_0$. Now we observe that $\lambda^*(s,\eps)$ is decreasing in $\eps$, i.e., it becomes larger as $\eps$ becomes smaller. to be continued.%On the other hand, the term $\Delta_{\le -1}(\eps,\lambda)$
% \end{proof}


% \begin{theorem}\label{thm:positive}
% positive result
% \end{theorem}

% \begin{proof}
% Not sure how to translate positive drift of $Z^t$ into runtime, since $\lambda^*$ changes over time, but here is one way. Probably split the process into intervals where $\lambda^*$ increases by a factor $1+\gamma$ in each interval. Then the $\lambda^*$ at the beginning of the interval gives positive drift throughout the whole interval, so we reach the end of interval. In a second phase, $\lambda$ increases to $\lambda^*$ of the end of the interval. Breals at the very end of the process since the intervals get small in terms of $Z^t$-distance, but once we have $\lambda^* \gg \log n$ we can completely neglect the negative drift.
% \end{proof}


% \ML{Here I put some stuff, which I believe will be useful.}

% % \begin{theorem}
% %     There exists \(F = 1 + o(1)\), constants \(0 < \delta < \varepsilon\) and \(0 < s, C\) such that the following holds. Consider the \saolea with initial search point \(\xinit \) satisfying \(\ZM(\xinit) = (\varepsilon \pm \delta) n\) and \(\linit = 1\). \ML{Should work for any \(\linit = o(n)\).} Then,
% %     \begin{enumerate}[(i)]
% %         \item the optimum is found in \(O(n)\) generations w.h.p.\ if \(f = \OM\); \ML{because we'll have concentration of \(\lambda\) we can probably also have some bound on the number of evaluations.}
% %         \item the optimum is found in \(e^{\Omega(n)}\) \ML{Maybe not correct exponent.} generations w.h.p.\ if \(f = \ADBV\).
% %     \end{enumerate}
% % \end{theorem}


% % \begin{definition}[Potential Function]
% %     We define 
% %     \begin{align*}
% %         h(\lambda) = -K \min\{0, \log_F( \lambda / n )\},
% %     \end{align*}
% %     with \(K\) a constant to be fixed later and 
% %     \begin{align*}
% %         g(x, \lambda) = \ZM(x) + h(\lambda).
% %     \end{align*}
% % \end{definition}

% % For conciseness, we will write \(Z^t = \ZM(x^t)\), \(H^t = h(\lambda^t)\) and \(G^t = Z^t + H^t = g(x^t, \lambda^t)\).

% \begin{lemma}
%     When \(f = \OM\) or \(f = \DBV\), we have asymptotically 
%     \begin{align*}
%         \lambda^*(\varepsilon n, s) = \Theta \left( \frac{1}{\varepsilon(s + 1)} \right).
%     \end{align*}
% \end{lemma}

% \begin{definition}
%     Let \(\delta > 0\) be a small constant. For \(f \in \{\OM, \DBV\}\), we define 
%     \begin{align*}
%         \tilde{\varepsilon}(s, \delta) := \inf \{\varepsilon > 0 \mid \Delta_1 + (1 + \delta) \Delta_{-1} > 0  \}.
%     \end{align*}
%     Additionally, we let \(\tilde{\lambda}^*(s, \delta) = \lambda^*( \tilde{\varepsilon}(s) n, s )\).
% \end{definition}

% \begin{lemma}
%     Let \(\delta > 0\) be a small constant and \(f \in \{\OM, \DBV\}\). Then \(\tilde{\varepsilon}(s, \delta)\) is well-defined, decreasing with \(s\). Additionally, \(\tilde{\lambda}^*(s, \delta)\) is increasing with \(s\) and satisfies asymptotically 
%     \begin{align*}
%         \tilde{\lambda}^*(s, \delta) = \Theta_\delta ( \log (s+1) ).
%     \end{align*}
% \end{lemma}


% \begin{proposition}
%     Let \(F = 1 + o(1)\) \ML{figure what \(F\) we want}. There exist constants \(0 \le \delta < \varepsilon \le 1/2\) and \(0 < s, \gamma, \eta\) such that the following holds. 
% \begin{enumerate}[(i)]
%     \item let \(f = \OM\), \(\ZM(x^t) \le (\varepsilon + \delta) n\) and \(\lambda^t = (1 \pm \gamma) \lambda_f(x^t) \), then 
%         \begin{align*}
%             \EE\left[ Z^{t} - Z^{t+1} \mid x^t, \lambda^t \right] \ge \eta;
%         \end{align*}
%     \item let \(f = \BV\), \(\ZM(x^t) = (\varepsilon \pm \delta) n\) and \(\lambda^t = (1 \pm \gamma) \lambda_f(x^t)\), then 
%         \begin{align*}
%             \EE\left[ Z^t - Z^{t+1} \mid x^t, \lambda^t \right] \le - \eta.
%         \end{align*}
% \end{enumerate}
    
% \begin{lemma}
%     Let \(f \in \{\OM, \ADBV\}\), \(F = 1 + o(1)\) and \(0 < \varepsilon, \gamma, s\) three constants. Assume that \(\linit = 1\) and \(\ZM(\xinit) \le \varepsilon n\). Define let \(T\) be the first time \(t\) at which \(\lambda^t = (1 \pm \gamma) \lambda_f(x^t)\). Then \(T  = o(n)\) with high probability.
% \end{lemma}

% It will be convenient to define \(Z^t_* = \min_{t' \le t} \{ Z^{t'} \}\) as the best value of \(\ZM\) observed so far. 

% \begin{lemma}
%     Let \(f \in \{\OM, \ADBV\}\), \(F = 1 + o(1)\) and \(0 < \varepsilon, \gamma, s\) three constants. Assume that \(\linit = 1\) and define let \(T\) be the first time \(t\) at which \(\lambda^t > (1 + \gamma) \lambda_f(Z^t_*)\). Then \(T = e^{\Omega(n)}\) with high probability.
% \end{lemma}

    
% \end{proposition}


==> technical.tex <==
\section{Technical Definitions and Results}
